Weakly Supervised Learning of Nuanced Frames for Analyzing Polarization in News Media

In this paper we suggest a minimally-supervised approach for identifying nuanced frames in news article coverage of politically divisive topics. We suggest to break the broad policy frames suggested by Boydstun et al., 2014 into fine-grained subframes which can capture differences in political ideology in a better way. We evaluate the suggested subframes and their embedding, learned using minimal supervision, over three topics, namely, immigration, gun-control and abortion. We demonstrate the ability of the subframes to capture ideological differences and analyze political discourse in news media.

==> 1Introduction.tex <==
\section{Introduction}\label{sec:introduction}
% \begin{itemize}
%     \item online content is highly biased and reflects different ideological and political perspectives
%     \item these perspectives are reflect both in the content of the articles, but also in the engagement patterns of users that interact with this content.
%     \item an extreme example is the formation of echo-chambers, or a ``softer verrsion'', users form communities. We expect these communities to capture shared interests, social relationship, and other properties users have in common. 
%     \item the community reflect both social and linguistic homophily. We evaluate both aspects.
%     \item our technical goal is to learn an embedding space connecting users and documents. We define communities as a probability distribution over a set of clusters. 
%     \item the embedding space captures both social, political and linguistic information, all of which is reflected in the community assignment.
%     \item 
% \end{itemize}

Over the last decade an increasing number of people access news online~\cite{Mitchell2016}, and use social networking platforms to engage, consume and propagate this content in their social circles. Social networks provide easy means to distribute news and commentary, resulting in a sharp increase in the number of media outlets~\cite{ribeiro2018media}, representing a wide range of perspectives and ideologies. However, despite this diversity, content is often shared only among people that hold similar beliefs and ideologies, resulting in highly segregated information communities, often referred to as \textit{``echo chambers''}~\cite{gentzkow2011ideological,quattrociocchi2016echo,dubois2018echo,garimella2018political}. 
%
To date, most works studying this phenomenon have either focused on the linguistic aspects of biased and polarized content~\cite{choi2012hedge,recasens2013linguistic,fulgoni-etal-2016-empirical,demszky2019analyzing}, \textit{or} on the social aspects connecting users to content providers and the way documents spread~\cite{volkova2017separating,glenski2018identifying,ribeiro2018media,li2019encoding}. Our main observation in this paper is that modeling both these aspects is needed in order to understand and analyze information communities.
%focused on analyzing the interactions between news sources and users in social networks~\cite{volkova2017separating,glenski2018identifying,ribeiro2018media}
%
Our goal in this paper is to formalize the connections between the perspectives expressed in the text, the users who share them, their social interactions and the information communities emerging from these connections. We suggest a novel, minimally supervised, approach for embedding information communities, which allows us to map the news media landscape on politically divisive issues, and capture the ideological biases and perspectives expressed in news content. We analyze the differences between communities based on their position on a continuous conservative-liberal ideological spectrum~\cite{ellis2012ideology,preoctiuc2017beyond}, and observe the differences in perspectives expressed in documents shared in these communities in three issues--  immigration, gun-control and abortion.
 
%
%Identifying the perspective difference and making it explicit can help strengthen trust in the newly-formed information landscape and ensure that all perspectives are represented. It can also help lay the foundation for the automatic detection of false content and rumors and help identify information echo-chambers in which only a single perspective is highlighted. %ribeiro2018media 


\subsection{Issue-Framing and Political Perspective}

To help clarify our objectives, consider two articles on the highly polarized immigration issue. \vspace{3pt}\\
%
\noindent\textbf{Example 1:}\textit{ Different Perspectives on Immigration}
 %Difference in frame usage by party. Topic: Immigration, Frame used: Economic
% colback=blue!5!white,colframe=blue!75!black
 
\begin{tcbraster}[raster columns=1,raster equal height,size=small, colframe,toprule=0pt, bottomrule=0pt, leftrule=0pt, rightrule=0pt, titlerule=0pt, arc=0pt]
\begin{tcolorbox}[colback=blue!15!white,colframe=blue!75!black,nobeforeafter, title={ \textit{Adapted from} \bf{Alternet }}~~(\textit{Left})]
  \small{{% These undocumented workers pay taxes for benefits they can't even use, like Social Security and Medicare. They also aren't eligible for benefits like the income tax credit.
%  A larger and more diverse population supports more intensive development of the resources available (...), leading, over time, to a steadily more prosperous national economy.
%
%Vox: Undocumented workers fund public schools and local government services by paying sales and property taxes like everyone else. The Institute on Taxation and Economic Policy estimates \$11.7 billion a year.
Employees-many of whom are undocumented immigrants from Mexico, Ecuador and elsewhere-toil seven days a week for less than minimum wage, with no overtime pay or sick leave.
% If undocumented migrants are prevented from
% entering and taking on farm work, and Americans won't do those jobs, what will happen to the nation's farms that rely on undocumented laborers?
}}
\end{tcolorbox}  
\begin{tcolorbox}[colback=red!15!white,colframe=red!75!black,nobeforeafter, title={ \textit{Adapted from} \bf{Breitbart }}~~(\textit{Right})]
  \small{{
% The editors of the Washington Post are finally admitting that high levels of legal immigration drive down wages for American workers, as President Trump has asserted.
Mass immigration has come at the expense of America's working and middle
class, which suffered from poor job growth, stagnant wages, and increased public costs to offset the importation of millions% of low-skilled foreign nationals.
  }}
\end{tcolorbox}  
\end{tcbraster}
\vspace{7pt}

The two articles capture opposite political perspectives, liberal (top) and conservative (bottom). They do not directly contradict each other, rather they focus the discussion on different aspects helping them argue their case. The first emphasizing the contribution of immigrants to the community through tax revenue, and the second emphasizing implication on wages for U.S. workers. This process is known as \textit{framing}~\cite{entman1993framing, chong2007framing}. 
%
Our goal is to both capture the political perspective associated with articles, and explain that perspective by identifying the framing dimensions in the text, which are associated with that perspective and support it. Previous work by~\citet{boydstun2014tracking} studied policy issue framing on news media and suggested 15 broad frames to analyze how issues are framed, which include \textit{Economic, Morality} and \textit{Security}, among others. These framing dimensions can help capture ideological splits~\cite{johnson2017ideological}. For example, by framing the immigration issue using the morality frame or using the security frame, the reader is primed to accept the liberal or conservative perspectives, respectively. However, as shown in Example 1, in some cases this analysis is too coarse grained, as both articles frame the issue using the economic frame, suggesting that a finer grained analysis is needed to capture the differences in perspective. To help resolve this issue, we suggest a data-driven refinement to these frames, described in section~\ref{sec:modelingFrames}, by identifying repeating expressions used in the context of the different frames, and grouping them to form \textit{sub-frames}, which can separate between different usages of the frame to express different political perspectives (e.g., \textit{Tax Revenue} vs. \textit{Salary Stagnation}).
%
 Our goal is to capture the ideological perspective associated with documents, identify how issues are framed to support these perspectives, and represent the political meaning of these frames on an ideological spectrum.
 

 \subsection{Embedding Information Communities}
 %Identifying political perspectives is typically framed as a text-categorization
The analysis discussed above is typically framed as text classification, e.g., biased language analysis~\cite{greene2009more, klebanov2010vocabulary, recasens2013linguistic}, political ideology identification~\cite{iyyer2014political, johnson2016all} or framing analysis~\cite{baumer2015testing,johnson2017ideological,hartmann2019issue}. Given the highly dynamic nature of political events and the strategies used to discuss them, these methods would require continuous adaptation.
%

Instead, we take a different approach driven by the principal of \textit{social homophily}~\cite{mcpherson2001birds}, referring to the tendency of individuals to form social ties with others who share their views. This phenomenon was previously used to help overcome language variation issues~\cite{yang-eisenstein-2017-overcoming}. In our settings, we follow the observation that the political perspectives and attitudes expressed in the text will be reflected in the behavior of users engaging with it. We identify similar patterns and exploit distant supervision to construct \textbf{information communities} consisting of documents and users,  holding similar views and focusing on similar aspects of the issues. Figure~\ref{fig:information_graph} describes an example for the immigration issue. 

We define the communities over an information graph, modeling the interaction between news document nodes, users who \textit{share} them on Twitter, and political influencers, such as politicians, \textit{followed-by} the sharing users.
%
%Given a graph connecting Twitter users nodes, via activity-links to news article nodes  (\textit{share}), and  via social-links (\textit{follow}) to politically affiliated users (e.g., Twitter accounts of members of Congress), 
Our algorithm groups users and news-article nodes together into communities, associates political meaning with these communities by observing the social links to politicians, and identifies repeating themes and perspectives by observing how the topic is framed in the news articles associated with each community.
%TODO: explain - the embedding space, allowing them to share representation, creates a common language for evaluating the relationship between these elements, connecting frames with political labels, documents (i.e., doc classification).  A community defines a probability distribution, over these elements, to belong to the same cluster. The assignments are overlapping.  The community is represented using its centroid, allowing us to create an embedding for the community, that can be evaluated in the embedding space - by observing its similarity with other elements, such as labels, and perspectives, which  explain that community. 
%
\begin{figure}[t!]
\centering
  \includegraphics[width=.77\linewidth]{Figures/network.pdf}
  \caption{Information Communities (Immigration)}
  \vspace{-10pt}
  \label{fig:information_graph}
\end{figure}
%
To accomplish that, we define a latent space for embedding users, documents, political influencers, frames and ideology-labels. Intuitively, the embedding space is shaped both by the textual content of documents, the engagement patterns of users with these documents and their social ties to politicians.  We take a community embedding approach~\cite{cavallari2017learning}, and define communities as a multivariate Gaussian distribution over that latent space. We suggest an EM-style learning approach, augmenting the graph embedding objective, based on first-order graph relations, with a global-view derived from the inferred community assignments.

Unlike related work analyzing community behavior and conflicts~\cite{kumar2018community,flores2018mobilizing,cunha2019all}, we do not analyze observed community structures, but rather our goal is to construct these communities, as a way to characterize how different issues are discussed and align social information with the text. Recent work by ~\citet{li2019encoding} exploits social supervision for detecting political bias in documents. We take a broader view in this work, and aim to characterize the discussion, rather than individual articles.


%TODO - what are our experiments designed todo?  One practical thing is to evaluate document classification, and show that adding communities can help.  More broadly - (1)  sanity check for the communities. (2) communities properties.
We conduct extensive experiments to evaluate the inferred community structures, over three politically divisive issues, namely, immigration, abortion and gun-control. We show that our approach can be used to detect the political ideology of documents, even when little social information is available, as well as characterize cohesive information communities, focusing on different aspects of these issues.


% (..TODO.. add discussion about frame refinement, community evaluation,)

% TODO : discuss disconnected docs

% todo: discuss "beyond binary labels" 

% todo : discuss the no-supervision settings - similar to topic models etc.



%Eval:

%Extenral Indicators of sanity -
% frame/subframe label correlation+visualization
%indicator correlation.
% classifier results - subframes are good features, comparable to BERT.



%Internal Sanity check -
%(What do SF mean) took top-K articles for each SF, and evaluated (Human) that they correspond to the definition (compared embedding with G-LDA).
% TODO: add example for a couple of paragraphs.
% (Can the embedding model classify) Sample 10 from each side, for each topic = 60 documents. Compare two lists of SF predicted from the text - GLDA vs. embedding



%Applying SF for analyzing data -
%event based table 

==> 3Modeling.tex <==
% \section{Social and Linguistic Modeling}\label{sec:modeling}
% In this section we first, define the social network context, on which we want to find politically polarized communities which are infused by language and, Secondly, we propose an Expectation Maximization Approach to identify politically polarized communities of Twitter users by embedding the social network interactions in a embedding space.



%\begin{figure*}[ht]
%\centering
%  \includegraphics[width=0.79\linewidth]{Figures/subframes.pdf}
%  \caption{Subframes identified by topic with percentage of articles containing the subframe in brackets.}
%  \label{fig2}
%\end{figure*}

% \paragraph{Data Collection}

\section{Data Collection }
 We collected 21,645 news articles on three highly polarized political topics, \textit{abortion, immigration} and \textit{gun control}. We used the hyper-partisan news dataset\footnote{https://pan.webis.de/semeval19/semeval19-web/} and collected additional documents on these topics from sources with known political perspectives based on the ranking provided by \url{mediabiasfactcheck.com}. We identify the topic of news articles by looking at presence of certain keywords in the titles and urls of news articles. For example, 'Abortion' for topic \textit{Abortion}; 'Migrant', 'Migration' for topic 'Immigration' etc. The hyper-partisan news dataset provides labels of the news articles and we labeled the rest of the news articles based on their media bias according to \url{mediabiasfactcheck.com}. We consider only the left and right biased news articles. The details of the collected data is summarized in Table x.
 %
%  We collected these articles by topic from news outlets with renowned political bias. In case of unavailability of reasonable amount of articles we supplement some news articles from Hyperpartisan news corpus. We identify the topic of news articles by looking at presence of certain keywords in the titles and urls of news articles. For example, 'Abortion' for topic \textit{Abortion}; 'Migrant', 'Migration' for topic 'Immigration' etc. We labeled the news articles based on their media bias according to \url{mediabiasfactcheck.com}.%\footnote{https://mediabiasfactcheck.com/}.
 We collected social information consisting of Twitter user handles that shared the news articles. To avoid news aggregators and inactive users we avoid users sharing more than $100$ or less than $5$ news articles. We identified follow relations instances between these users and members of the U.S. Congress and Senate.
  The dataset is summarized in Table \ref{tab:dataset-summary}. Note that the majority of documents are \textbf{not} shared on social media, simulating a realistic setting, where social supervision is only partially available. 
  

 

% \begin{table*}[ht]
% \centering
% \scalebox{0.82}{
% \begin{tabular}{>{\arraybackslash}m{4cm}|>{\centering\arraybackslash}m{4cm}|>{\centering\arraybackslash}m{4cm}|>{\centering\arraybackslash}m{4cm}}
%  \hline
%  & \textbf{Abortion} & \textbf{Gun Control} & \textbf{Immigration} \\
%  \hline
%  No. of News Articles & 6,476 (L: 3,437, R: 3,039) & 6,653 (L: 3,198, R: 3,455) & 8,516 (L: 3,496, R: 5,020)\\
%  Shared on Twitter & 2,116 (L: 1,011, R: 1,105) & 2,243 (L: 962, R: 1,281) & 4,238 (L: 2,187, R: 2,051)\\
%  Not Shared on Twitter & 4,360 (L: 2,426, R: 1,934) & 4,410 (L: 2,236, R: 2,174) & 4,278 (L: 1,309, R: 2,969)\\
%  \hline
%  No. of Politicians & 568 (L: 301, R: 267) & 568 (L: 301, R: 267) & 568 (L: 301, R: 267)\\
%  No. of Twitter Users & 4,094 & 3,257 & 10,374\\
%  No. of Follow Relation & 64,344 & 51,707 & 178,060\\
%  No. of Share Relation & 40,197 & 22,762 & 132,760\\
%  \hline
% \end{tabular}}
% \caption{Dataset Summary. L and R means Left and Right Bias respectively.}
% \label{tab:dataset-summary}
% \end{table*}


\begin{table*}[ht]
\centering
\scalebox{0.75}{
\begin{tabular}{>{\arraybackslash}m{3.5cm}|>{\centering\arraybackslash}m{4.5cm}|>{\centering\arraybackslash}m{4.5cm}|>{\centering\arraybackslash}m{4.5cm}}
 \hline
 & \textbf{Abortion} & \textbf{Gun Control} & \textbf{Immigration} \\
 \hline
 News Articles & 6,476 (L: 3,437, R: 3,039) & 6,653 (L: 3,198, R: 3,455) & 8,516 (L: 3,496, R: 5,020)\\
 Shared & 2,116 (L: 1,011, R: 1,105) & 2,243 (L: 962, R: 1,281) & 4,238 (L: 2,187, R: 2,051)\\
 Not Shared & 4,360 (L: 2,426, R: 1,934) & 4,410 (L: 2,236, R: 2,174) & 4,278 (L: 1,309, R: 2,969)\\
 \hline
 Politicians & 568 (L: 301, R: 267) & 568 (L: 301, R: 267) & 568 (L: 301, R: 267)\\
 Users (Follow) (Share)  & 4,094 (64,344) (40,197) & 3,257 (51,707) (22,762) & 10,374 (178,060) (132,760)\\
%  No. of Follow Relation & 64,344 & 51,707 & 178,060\\
%  No. of Share Relation & 40,197 & 22,762 & 132,760\\
 \hline
\end{tabular}}
\caption{Dataset Summary. L and R means Left and Right Bias respectively.}
\label{tab:dataset-summary}
\end{table*}



% \begin{figure}[ht]
% \centering
%   \includegraphics[width=1\linewidth]{Figures/framing-example-new.pdf}
%   \caption{Difference in frame usage by party. Topic: Immigration, Frame used: Economic}
%   \label{fig2}
% \end{figure}

\section{Modelling Political Framing}\label{sec:modelingFrames}

Political framing~\cite{entman1993framing,chong2007framing}  is a nuanced political strategy, used to bias the discussion on an issue towards a specific stance by emphasizing specific aspects of the issue priming the reader to accept that stance. In Example 1, the discussion around the topic of immigration can be framed around the tax revenue from immigrant work, a pro-immigration perspective associated with the left, or the stagnating wages of U.S. workers, a perspective associated with the right. Using framing to analyze political discourse and news media has gathered significant interest over the last few years~\cite{tsur2015frame, card-EtAl:2015:ACL-IJCNLP, baumer2015testing,johnson2017ideological,field2018framing,morstatter2018identifying,ajjour-etal-2019-modeling,liu-etal-2019-detecting,hartmann2019issue}. The frames used for this analysis could be issue specific (e.g., the mental-health of the shooter, when analyzing tweets about gun-violence events~\cite{demszky2019analyzing}), or as suggested by \citet{boydstun2014tracking}, generalize over several policy issues, using a fixed set of frames, e.g., framing immigration as a \textit{security, fairness}, or \textit{economic} issue. %The same dimensions can be used for analyzing other topics as well.  

The tradeoff between issue-specific frames and general policy frames is clear. The first approach is tailored for the specific nuances of each topic, capturing a direct relationship between framing strategies and political stance, while the second does not require a close familiarity with the topic, and generalizes across topics.
%
In many cases, as we show in this paper, using policy frames does not capture the nuanced aspects of the issue highlighted by each side to bias the discussion. In Example 1, both sides use the \textit{economy} frame, however it is instantiated in different ways, to promote opposite views.  To help combat this issue, we suggest a middle ground between generalized policy frames and event-specific frames, by constructing a hierarchy of frames and sub-frames, the first derived from the definitions and data of the media
frames corpus~\cite{card2015media}, and the second emerging from the data directly, by tracking the differences in the vocabulary used when these frames are instantiated in our dataset. We associate political meaning with the sub-frames by embedding them in a shared space with political information, as described in Section~\ref{sec:inference}.
%
This process follows two steps.

% \cite{johnson2017ideological} showed that politicians on Twitter emphasize on different things to induce their ideology regardless of using the same frame by using different ideological phrases. We attempt to analyze the same phenomenon in case of news articles. For example let's look at the examples in Figure \ref{fig2}. In (a), both of the text snippets use the frame 'Economy' but emphasize on different things. In the first snippet, the right wing news outlet emphasizes on the job scarcity of Americans because of mass immigration while the second snippet from the left wing outlet says immigrants are needed for farm work. Similarly, in (b), both snippet frames abortion from 'Morality and Ethics' perspective. But the right wing emphasizes on evil of abortion while left wing says opposing abortion is rooted from the intention of controlling women.
% So, we hypothesize that the emphasis on aspects will be different by parties regardless of using the same frame. So, we identify most used bigrams and trigrams when framing an issue by each of the $15$ Policy Frames. This process requires following teo steps.

\noindent\textbf{Step 1:} \textit{Annotate news articles paragraph with policy frames}. We follow the procedure suggested by \citet{field2018framing}, and use the media frame corpus to derive a unigram lexicon for each of the $15$ frames based on their Pointwise Mutual Information (PMI) \cite{church1990word}. We use the $250$ top-PMI words for each frame. This lexicon is used to annotate paragraphs of new articles by ranking frames by the number of lexicon matches, and using the top-2 frames. We discard unigrams occuring in  $<0.05\%$ and $>98\%$ of the documents.

\noindent\textbf{Step 2:} \textit{Building Issue-specific Lexicons.} The annotated paragraphs are used to create issue-specific lexicons, which capture the nuanced ways in which frames are used. We construct a bi-gram and tri-gram lexicon for each frame by calculating the PMI for each frame and each bi-gram and tri-gram in the corpus and using the top PMI ones.  We did not consider bi-grams or tri-grams occuring in $>50\%$ and $<0.02\%$ of the paragraphs. The process is issue-specific, resulting in three lexicons, ones for each issue we study in this paper. Following this procedure we found $4,082$ bigrams and $1,669$ trigrams for the topic \textit{Abortion}, $3,293$ bigrams and $1,451$ trigrams for the topic \textit{Gun Control}, $3,743$ bigrams and $1,385$ trigrams for the topic \textit{Immigration}.

% \noindent\textbf{Step 2:} \textit{Building Frame Specific Bi-gram and Tri-gram Lexicon: } Now, after annotating each paragraph with top-2 frames, we build lexicons of bi-grams and tri-grams for each frame using the same PMI based approach. We calculate the PMI between each frame and each bi-gram and tri-gram in the corpus and construct a new frame lexicon with the highest PMI score. We didn't consider bi-grams or tri-grams apprearing more than $50\%$ of the paragraphs and less than $0.02\%$ of the paragraphs. For an n-gram $g$ we calculate the pointwise mutual information with frame $f$, $I(g, f)$ using the following formula.
% \begin{align*}
%     I(g,f)=\operatorname{log}\frac{P(g|f)}{P(g)}
% \end{align*}{}
% Where $P(g|f)$ is computer by taking all paragraphs annotated with frame $f$ and computing $\frac{count(g)}{count(allngrams)}$ and similarly, $P(g)$ is computed by counting ngram $g$ over the whole corpus. We, assign each n-gram to the frame class with highest PMI score and build an n-gram lexicon for each frame. Note that, these lexicons are topic specific which means we don't mix up documents from various topics while building these lexicons. Every topic gets its own frame specific lexicons. Following this procedure we found 4,082 bigrams and 1,669 trigrams for the topic \textit{Abortion}, 3,293 bigrams and 1,451 trigrams for the topic \textit{Gun Control}, 3,743 bigrams and 1,385 trigrams for the topic \textit{Immigration}. \\

The issue-specific lexicon is designed to break the way each frame is used, such that different aspects-of and perspectives-on, the issue can be captured. Instead of using this lexicon directly, we add the lexicon into our information-map. Each sub-frame n-gram expression defines a node, connected via edges to documents in which it appears. The importance of embedding this information is two-fold: (1) it helps shape the learned communities, complementing the social information, as we hypothesize that phrase usage will be different based on political affiliation; (2) it provides the means to connect unshared  documents, without  social information, to the graph and propagate the social supervision to these document nodes.\\
\textbf{Sub-frames Construction} We hypothesize that the sub-frames n-grams lexicon captures the different perspectives underlying the way frames are instantiated in articles, and the views of users who engage with them. To help evaluate this property, we group the n-gram phrases for each frame into several groups, each group capturing a specific aspect of the issue. This grouping followed known political talking points, extracted from \url{www.ontheissues.org},  on the three topics (\textit{Abortion, Immigration and Gun Control}),  and was validated based on the documents the phrases appeared in. We refer to these groups as \textit{Sub-Frames}. The list of identified subframes is in Figure \ref{fig2}. The subframe title explains the talking point. %More details are provided in the Supplementary materials.

 

% We hypothesize that phrases capture ideological stances in news articles regardless of same frame usage. To prove this phenomenon and evaluate the linguistic homophily in the communities of Twitter users, we group the bi-gram and tri-gram phrases found in our framing analysis in several groups based on the possible aspect focused by them. We do this grouping by using known political talking points on the three topics - \textit{Abortion, Immigration and Gun Control}. We define this groups as \textit{Sub-Frames}. For example, consider the examples shown in Section \ref{sec:introduction}. We can ground the text segment from \textit{Vox} to the subframe 'Tax Revenue' because of the usage of the bigram 'pay taxes' and the text segment from 'Breitbart' to 'Salary Stagnation' because of the usage of the trigram 'drive down wages'. The list of identified subframes are shown in Table \ref{table2}. The subframe names explain their talking points. The details of the other subframes are attached in the Appendices.  


% The importance of the frame specific phrases lexicon in this project is two way- (1) We can form communities by inducing the phrase usage explicitly which is expected to yield cleaner communities as we hypothesize that phrase usage will be different based on political affiliation; (2) We can linguistically connect unshared news articles to the social network via frame specific phrases and propagate the social information to their embedding learning. This embedding learning is expected to be helpful in identifying the bias present in them and to resonate which communities will be interested in sharing those articles. Note that we can do that without using any direct supervision from the text, where the proposed approach by \cite{li2019encoding} fails to incorporate unshared document in their embedding learning. After identifying all of the bigrams and trigrams, we can embed those jointly in the graph embedding space. We define the set of all bigrams and trigrams as $G$.    

\begin{table*}[ht]
\begin{center}
 \scalebox{0.71}{\begin{tabular}{>{\arraybackslash}m{6.5cm}||>{\centering\arraybackslash}m{1.9cm}|>{\centering\arraybackslash}m{1.9cm}||>{\centering\arraybackslash}m{1.9cm}|>{\centering\arraybackslash}m{1.9cm}||>{\centering\arraybackslash}m{1.9cm}|>{\centering\arraybackslash}m{1.9cm}} 
 \hline 
\textsc{Frames} & \multicolumn{2}{c}{\textsc{\textbf{Abortion}}} & \multicolumn{2}{c}{\textsc{\textbf{Immigration}}} & \multicolumn{2}{c}{\textsc{\textbf{Gun Control}}}\\ [0.5ex]
\cline{2-7}
&   \textsc{Frame indicator}   &   \textsc{Subframe indicator}   &   \textsc{Frame indicator}   &   \textsc{Subframe indicator} &   \textsc{Frame indicator}   &   \textsc{Subframe indicator}\\
 \hline
 F1: Economic                                   & 0.95&   0.44&   0.92& 0.28&   0.94&   0.29\\
 \hline
 F2: Capacity and Resources                     & 0.95&   0.24&   0.89& 0.38&   0.92&   0.38\\
 \hline
 F3: Morality                                   & 0.91&   0.30&   0.89& 0.16&   0.93&   0.16\\
 \hline
 F4: Fairness and Equality                      & 0.93&   0.37&   0.92& 0.30&   0.93&   0.41\\
 \hline
 F5: Legality, Constitutionality, Jurisdiction  & 0.96&   0.54&   0.92& 0.46&   0.95&   0.39\\
 \hline
 F6: Policy Prescription and Evaluation         & 0.97&   0.58&   0.92& 0.07&   0.95&   0.48\\
 \hline
 F7: Crime and Punishment                       & 0.94&   0.36&   0.90& 0.32&   0.94&   0.61\\
 \hline
 F8: Security and Defense                       & 0.95&   0.17&   0.91& 0.28&   0.93&   0.41\\
 \hline
 F9: Health and Safety                          & 0.96&   0.43&   0.94& 0.13&   0.95&   0.48\\
 \hline
 F10: Quality of Life                           & 0.94&   0.34&   0.92& 0.37&   0.93&   0.19\\
 \hline
 F11: Cultural Identity                         & 0.93&   0.22&   0.88& 0.03&   0.93&   0.41\\
 \hline
 F12: Public Sentiment                          & 0.91&   0.33&   0.90& 0.05&   0.94&   0.42\\
 \hline
 F13: Political                                 & 0.94&   0.53&   0.93& 0.51&   0.96&   0.46\\
 \hline
 F14: External Regulation and Reputation        & 0.93&   0.22&   0.88& 0.18&   0.93&   0.51\\
 \hline
 F15: Other                                     & 0.94&   0.18&   0.92& 0.21&   0.93&   0.38\\
 \hline
 Overall                                        & 0.94 (0.017)&   0.35 (0.128)&   0.91 (0.018)& 0.25 (0.142)&  0.94 (0.011)&   0.40 (0.112)\\
 \hline 
 \end{tabular}}
\caption{}
\label{tab:purity}
\end{center}
\end{table*}


\begin{table}[ht]
\begin{center}
\scalebox{0.71}{
\begin{tabular}{>{\arraybackslash}m{4cm}|>{\centering\arraybackslash}m{1.7cm}|>{\centering\arraybackslash}m{1.7cm}|>{\centering\arraybackslash}m{1.7cm}}
 \hline
 Models & \textbf{Abort.} & \textbf{Imm.} & \textbf{Gun} \\
 \hline
 LR (Frame Indicators) & 74.57 (0.6) & 82.36 (0.6) & 70.62 (0.8)\\
 LR (Subframe Indicators) & 81.47 (0.2) & 85.31 (0.2)  & 72.34 (0.5) \\
 BERT & 81.58 (1.8) & 79.72 (3.7) & 73.21 (0.7)\\
 HLSTM & 81.12 (0.4) & 84.69 (1.7) & 71.08 (2.8) \\
 \hline
\end{tabular}}
\caption{Test F1 scores (standard deviation) of article classification task (left/right) using 3 fold cross validation. LR is for Logistic Regression with type of one hot encoded features in the brackets.}
\label{tab:dataset-summary}
\end{center}
\end{table}







==> 4Inference.tex <==
\section{Information Community Construction}\label{sec:inference}

% \begin{algorithm}
% \begin{algorithmic}[1]
% \Require Information Graph $G=(V,E)$
% \Ensure (1) $Emb_G$, an embedding of $G$'s nodes (2) $k$, the number of communities (3) $\pi_{ik}$, community membership probability, (4) community embedding parameters $\Psi_k$
% \State $Emb_G \Leftarrow Embed\_Graph(G) $\Comment{Initialize graph embedding}
% %

% % \State $X \Leftarrow x$
% % \State $N \Leftarrow n$
% \While{Stopping criteria not met}
%  \State Detect communities
%  \State Infer Ideology
%  \State Embed Graph
% % \If{$N$ is even}
% %   \State $X \Leftarrow X \times X$
% %   \State $N \Leftarrow \frac{N}{2} $  \Comment{This is a comment}
% % \ElsIf{$N$ is odd}
% %   \State $y \Leftarrow y \times X$
% %   \State $N \Leftarrow N - 1$
% % \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}
% What is a community? What is the input-output relationship of the community construction process. How does it answer questions of social-linguistic homophily? 
In the previous section we introduced several nuanced framing dimensions (i.e., \textit{sub-frames}), capturing how the general issue-frames decompose into topic-specific frames. Our next goal is to associate these frames with political meaning. Instead of a supervised learning approach, dealing with the text in isolation, we derive supervision from the social context in which the documents are shared and propagate this information to the identified frames.

% From a technical perspective, 
The input for this process is a graph, consisting of several node types -- documents, sub-frames denoting expressions (see Section~\ref{sec:modelingFrames} for an explanation), users sharing them, and political influencers with a known political affiliation. Our technical challenge is to propagate information from influencers to content nodes. Note that the majority of documents are not associated with social information, exacerbating the weak-supervision problem.

We address this challenge by interleaving between two steps. In the first, we learn a graph embedding~\cite{perozzi2014deepwalk,tang2015line,grover2016node2vec}, which aims to maximize the similarity between neighbouring nodes. This process allows label information to be propagated from influencers to sharing users and finally to articles and the sub-frames they use. In the second step, we detect communities in the graph ~\cite{leskovec2010empirical,xie2013overlapping,cavallari2017learning}, defined as overlapping clusters of users and content nodes that share perspectives, political ideology and are influenced by similar users. While community assignments are not directly observed, they are represented in the embedding space, and can be inferred from it. We use these inferences to augment the objective function of the graph embedding learning problem.


%users, documents they engage with, and the perspectives expressed in these documents. Formally, these communities are defined as soft clusters over the learned representation of these elements.

% \paragraph{Input and Output Definitions}
%  We refer to these elements using the following notation, $A$ is the set of news articles, $U$ is the set of Twitter users, $P$ is the set of politicians and $L$ is the labels associated with them (left and right).  $P$ and $U$ are disjoint. In section~\ref{sec:inference} we explain how these elements are embedded, specifically, how the political label information propagates from political users to the entire graph.

% \textbf{TODO }: Add frames and sub-frames to the graph defintion. 

\subsection{Information Graph Embedding}\label{sec:observed-relations}

We define the notion of information-landscape in which documents appear as an \textbf{Information Graph}, $G=(V,E)$, where V consists of several node types -- articles  $A$, Twitter users $U$, sub-frames expressions $SF$, political influencers (corresponding to politicians) $P$ and nodes indicating their bias, $L$ (i.e., liberal or conservative). Edges in $E$ connect nodes in $SF$ and $A$ based on the sub-frame expressions identified in the text, $U$ and $A$ via \textit{sharing} links, $U$ and $P$ via \textit{follow} links, and finally $P$ and $L$ based on their political affiliation.

We define an embedding function $\Phi$, mapping nodes in the graph to vectors in $\mathbb{R}^d$.  The embedding function correspond to neural architectures associated with the different node types and trained jointly to capture the graph relations (we provide more technical details below). Specifically, we construct positive instances for the embedding objective by associating each node $o$ with all its graph neighbours, and for each positive pair $(o,m^p)$, we sample 5 negative instances, $(o,m^n)$ such that $o$ and $m^n$ do not share an edge. Given all generated examples, we define the loss function as:
% Now given the set of politician nodes, $P$; Twitter user nodes $U$; label nodes, $L$; article nodes $A$, ngram nodes $G$, we can embed them jointly in an embeddings space based on their connection with each other following the technique proposed by \citet{li2017joint}. We can observe the following objectives to maximize from the graph - Politicians ($P$) connect to their Labels ($L$); Twitter users ($U$) connect to Politicians ($P$) they follow; News articles ($A$) connect to Twitter users ($U$) they are shared by; News articles ($A$) connect to ngrams ($G$) they contain. Now, given any node $o$, a positive example $m^{p}$ and a negative example $m^{n}$, where $o$ is connected to $m^{p}$ and $o$ is not connected to $m^{n}$, we can define the embeddings loss as follow,

{\footnotesize
\vspace{-5pt}
\begin{align*}
    %\operatorname{Bias}_{a}=\operatorname{arg\,max}_{b\in B} sim(a, b)
    %E_{r}(o,m^{p},m^{n})=
    E_r=l\Big(\operatorname{sim}(\Phi(o), \Phi(m^{p})), \operatorname{sim}(\Phi(o), \Phi(m^{n}))\Big)
\end{align*}\vspace{-2pt}
}
$E_{r}$ defines the embedding loss for a specific relation type $r$ (e.g, politicians to labels). %At most $5$ negative pairs were chosen randomly per positive pair. %Our goal is the maximize the similarity of a node embedding with a positive example and minimize the similarity with a negative example.
As, a similarity function, $sim()$, we use cosine similarity and $l()$ is cross-entropy loss, maximizing the similarity between the embedding of entities in positive examples (and minimizing it for negative pairs).

% which is defined as follows.
% \begin{align*}
%     l(p,n)=-\operatorname{log}(\frac{e^{p}}{e^{p}+e^{n}})
% \end{align*}
%
We minimize the sum of relational loss functions $\sum_{r \in R} \lambda_{r} E_{r}$, where $R$ is the set of relation types, and the weight $\lambda_{r}$ is associated with each type.\\
Node embedding are initialized randomly, except article nodes that use a Hierarchical-LSTM \cite{hochreiter1997long}. We run an LSTM, using Glove \cite{pennington2014glove}, over each sentence words, and average the hidden states to represent sentences. Then, a second LSTM is used over the embedding of sentences, our final representation averages its hidden states. The HLSTM is trained jointly with the embedding.

\noindent\textbf{Inference: }We can infer the bias $l\in L$ of any node $a$, using:
%
% \begin{align*}
~{\small $\operatorname{Bias}_{a}=\operatorname{arg\,max}_{l} sim(\Phi(a), \Phi(l))$}
% \end{align*}


\subsection{Detecting and Embedding Communities}\label{sec:detected-relations}%{EM Approach for Community Detection}
%motivation for communities.
%what are communities formally - GMM, what are the parameters we associate with learning it.
%How to interpret communities - "inference over the embedding space", both for "real" nodes and for centriod nodes representing the communities. 
In the next step we identify structure in the information graph and use it to augment the embedding learning objective, which focuses on local relations, with global structural information. We hypothesize that Twitter users with similar social behaviour and common interests and perspectives (exhibited in the news articles they share) can be grouped together to form an \textit{information community}.

We define communities as overlapping clusters by using a Gaussian Mixture Model (GMM), defined over the nodes' embedding. We follow~\citet{cavallari2017learning} and define the embedding for community $k\in\{1,...,K\}$ as a multivariate Gaussian distribution $\mathcal{N}(\psi_k,\Sigma_k)$, where $\psi_k\in \mathbb{R}^d$ is the mean vector and $\Sigma_k$ is the co-variance matrix. Given these parameters, we can define $\pi_{ik}$ as the $k$-th community membership probability for the embedding of graph node $i$.  We exploit the fact that $\pi_{ik}$ captures global structure, not observed directly via edges, and encode community membership as additional supervision for the embedding function. %We treat the community mean vector $\psi_k$ as the community representation, and associate additional properties to the community members based on 

Since community memberships are not known, we estimate them using an EM-style approach, in which node embedding, community embedding and membership are learned jointly, by iterating between three major steps described in Figure \ref{fig:em}.
% which exhibits an information echo-chamber in both social and textual dimensions. We attempt to capture these latent community structures in our graph. When we have identified these latent community structures, we can infer various social and textual properties of these latent communities. Then we can induce the embedding learning with newly inferred objectives which is expected to improve the quality of the learned embeddings. For this we propose a noble EM style approach as described below.\\
%Our approach is inspired from the approach proposed by \citet{cavallari2017learning}. They propose a closed loop EM-approach to learn community and node embeddings jointly by influencing the embeddings of nodes and communities by each other. Our approach can be divided into three major steps as shown in Figure \ref{fig:em}.

\begin{figure}[h]
\centering
  \includegraphics[width=0.85\linewidth]{Figures/EM_1.pdf}
  \caption{Community Embedding Approach}
  \label{fig:em}
\end{figure}

\textbf{(1) Initial Belief Step } We define $S_{IG}$ as the learning objective derived from the information graph, described in Section \ref{sec:observed-relations}. Two additional objectives, $S_{C}$ and $S_{L}$ are initialized to $\emptyset$

\textbf{(2) Step 1: }  In this step we learn a graph embedding, described in Section \ref{sec:observed-relations}, using the three objective functions,  $S_{IG}$, $S_{C}$ and $S_{L}$ (the latter are explained in Step 2 of the algorithm). The result of this step is a graph embedding function $\Phi$.

% We learn the embeddings of each node following the procedure described in Section \ref{sec:observed-relations} using learning objectives $S_{known}$.
\textbf{(3) Step 2: } In this step we identify communities of Twitter users and populate $S_{C}$ and $S_{L}$, based on inferred information.  Given the learned embedding function $\Phi$, we cluster the sharing users ($U$ nodes). 
%Given we have learned the embeddings of all of the users, we can find the cluster of the Twitter users using Gaussian Mixture Model (GMM) \cite{bishop2006pattern}. 
We consider the embedding $\Phi(u_i)$ of a Twitter user as generated by a multivariate Gaussian distribution from a community $c_i = k$. We obtain the community embedding (i.e., GMM parameters) and community assignments, by maximizing the likelihood of the data, defined over the embedding space.
{\small
$$\prod_{i=1}^{|U|}{\sum_{k=1}^{K}{p(c_i=k)p(\Phi(u_i) |c_i=k, \Psi_k, \Sigma_k)}}$$}
where $p(c_i = k)$ is the probability of user $i$ belonging to community $k$, $\Psi_k$ and $\Sigma_k$ are mean vector and co-variances matrix for community $k$. 
%
Since the number of communities $K$ is not known, we  dynamically determine it at each iteration using the Bayesian information criterion (BIC) score \cite{schwarz1978estimating}. We take the number of communities at the BIC score knee point that is above a threshold $t_{n}$ (determined empirically).\\ %TODO- @Shamik - what is the threshold you used?
%of BIC scores beyond which point the BIC score becomes almost constant. 
%
\indent\textbf{Exploiting the Community Structure} The community membership provides us with additional information, used to improve the learned node representation. We define two new objectives, $S_C$, using the community assignments, and $S_L$ inferring the political bias of users and articles.


% \noindent(1) \textit{Twitter users to community centroid: } 
\noindent(1) \textit{Encouraging Cohesiveness using Community Assignments}. Our first objective, $S_C$, is designed to project the community assignments to the embedding space. We represent a community $k$ in the embedding space using its mean vector $\Psi_{k}$. We use the community membership probability $\pi_{ik}$ to define the embedding objective, by maximizing the similarity between a user $i$ and the community centroid $k$ for which $\pi_{ik}$ is maximized. Given the users assignments, we add articles shared by them as additional instances, maximizing the similarity between them and the assigned community centroids. We sample 5 negative examples for each added example. The added examples bias $\Psi$ to learn \textit{cohesive} representations for documents and users mapped to the same community.
%@Shamik-did you also add negative examples?
 

% Given the centroid embeddings of the communities ($\Psi_{k}$) and probability distribution for each Twitter user over all the communities ($P(c_{i}=k)$), we can define a objective function which maximizes the similarity between a Twitter user and his nearest centroids. We define the set of centroid nodes as $C$. The advantage of GMM is that it provides us with a probability distribution for each user over all possible communities. So, our model is flexible to incorporate soft community assignment i.e. one Twitter user can fall in multiple communities. Moreover, maximizing similarity with community centroids add high order proximity to our graph embedding learning in linear time complexity.

% After assigning Twitter users to communities we readily know the assignment of news articles to the communities as we know which news articles are shared by which user. So we can define an objective which maximizes the similarity between a news article and the centroid of the communities it is shared in.



% \noindent(2) \textit{Twitter users to Labels: } 
\noindent(2) \textit{Inferring Political Perspective.} The political perspective expressed in articles and endorsed by users sharing them is not directly observed in our setting. Instead, as explained in \ref{sec:observed-relations}, political perspective is represented in the embedding space, and can be inferred from it. We use this information, and maximize the similarity between sharing user nodes and the inferred label. After each iteration we update our beliefs on sharing users' labels.

While still ambiguous, the weak supervision signal from political users is less noisy when applied to sharing users, as the two are directly connected via edges. Articles rely on sharing users, which introduce additional noise, to propagate this information through the embedding space. As a result, we take a more prudent approach, and infer article labels by looking at their community assignments. We associate a political bias with each community, by comparing the similarity of its centroid with the embedding of each political perspective. We compare the number of times the article was shared in left-leaning vs. right-leaning communities, and use the majority's label for that article. The inferred labels are used to populate $S_L$ with  article (or user) and inferred label inferred, and use it to maximize their similarity in the embedding space.


% \noindent(4) \textit{News article to label: } We can make predictions about the labels of news articles by looking at their community assignments. 

% If a news article is shared in more left biased communities than right, it is predicted as a left biased article and vice versa. Note that we can determine the label of a community by using the inference rule defined in \ref{sec:observed-relations}. Then we maximize the similarity between news articles and predicted labels. We only make prediction about news articles which are shared in at least $2$ communities with a hope to minimize incorrect predictions. So, the labels of a subset of news articles are predicted at each step and we only update the predictions in previous E steps.\\
% So at each E step we discover and update the above set of new objectives. We define the set of discovered objectives as $S_{discovered}$. In the next, M step we learn the graph embeddings using $S_{known}\cup S_{discovered}$. 
% \paragraph{Output Communities: } After each E step, we check for the stopping criteria and decide if we need to perform the M step or not. For that, we look at the predicted labels of all news articles and Twitter users using the formula above. If in two consecutive E steps, the change in predicted labels of the articles and Twitter users is less than a threshold $t$, we stop our learning and return the communities.

%    \item \textbf{News articles to Community centroid: } After assigning sharing users to communities we assign the news articles they actually share to the same community and maximize the similarity between news articles and centroid. In case of an unshared news article we assign the news article to the nearest community in the embedding space. 
%    \item \textbf{Twitter users to Labels: } To keep an overall consistency in the embeddings learning process we determine the label of sharing users based on their similarity with labels and maximize the similarity between sharing user node and label in subsequent M step. Note that in each E step, we update our belief on the labels of sharing users.
%    \item \textbf{News articles to Labels: } After assigning news articles to communities, we can make predictions about their bias by looking at their community assignment. If a news article is shared in more left biased communities than right, it is predicted as a left biased article and vice versa. Then we maximize the similarity between news articles and predicted labels. We only make prediction about news articles which are shared in at least $2$ communities with a hope to minimize incorrect predictions. So, the bias of a subset of news articles are predicted at each step and we only update the predictions in previous E steps.


%The main difference of their approach with our is that in their learning the number of communities are known from prior. But in social network environment we do not know the exact number of communities. So, we break the closed loop of learning and during each expectation step we make prediction on possible number of communities and in the following maximization step we include this information as objective function for learning the embeddings. Which is the advantage of the open loop approach that we can discover new kind of learning objectives in expectation step and include them in following maximization step. Note that other state of the art community detection techniques like GCN \cite{kipf2016semi} fails in this aspect that they require the graph relation learning objectives and number of communities to be known completely from prior. Our EM-Approach is shown in Figure \ref{fig1}. The steps of learning embeddings and detecting communities are described below.



%\paragraph{(1) Initialization of Known (Observed) Objectives} We discover following relations from the social network.
%\begin{itemize}
%    \item \textbf{Politicians to Labels: } 
%    \item \textbf{Twitter users to Politicians: }
%    \item \textbf{News articles to Twitter users: }
%\end{itemize}{}
%Now, we can learn the embeddings of all the nodes using the social objectives. Following the procedure we are emphasizing only social network information. To infuse the representation of nodes by kind of stances expressed in the news articles, we add the following textual objectives based on our hypothesis that outlets cover different aspects of the same event based on their political bias. Moreover, articles which are not socially connected can be connected via their textual connections.
%\begin{itemize}
%    \item \textbf{News articles to Ngrams: }
%\end{itemize}{}

%\paragraph{(2) Learn Embeddings using Known Objectives} 

%\paragraph{(3) Identify Communities and Discover New Objectives} 
%After learning embeddings of all of the nodes we identify the communities of sharing users using their learned embeddings. We use Gaussian Mixture model \cite{bishop2006pattern} to find communities of sharing users. Note that we do not know the number of communities in prior. So, we dynamically determine the number of communities at each Expectation step by looking at the Bayesian information criterion (BIC) score. We take the number of communities at the knee point of BIC scores beyond which point the BIC score becomes almost constant. The mean of each Gaussian is considered as the centroid of each community and we can predict the label of each community by looking at the similarity score of centroid embedding and label embedding. After discovering the communities, we add the following embeddings learning objectives to our known objectives.

%\begin{itemize}
%    \item \textbf{Twitter users to Community centroid: } We embed the community centroids found. The mean of each Gaussian is the embeddings of the corresponding centroid. We maximize the similarity between Twitter users and the centroid of the community they fall in. The advantage of Gaussian Mixture Model is that it provides us with a probability distribution for each user over all possible communities. So, our model is flexible to incorporate soft clustering. Moreover, maximizing similarity with community centroids add high order proximity to our graph embedding learning in linear time complexity.  
%    \item \textbf{News articles to Community centroid: } After assigning sharing users to communities we assign the news articles they actually share to the same community and maximize the similarity between news articles and centroid. In case of an unshared news article we assign the news article to the nearest community in the embedding space. 
%    \item \textbf{Twitter users to Labels: } To keep an overall consistency in the embeddings learning process we determine the label of sharing users based on their similarity with labels and maximize the similarity between sharing user node and label in subsequent M step. Note that in each E step, we update our belief on the labels of sharing users.
%    \item \textbf{News articles to Labels: } After assigning news articles to communities, we can make predictions about their bias by looking at their community assignment. If a news article is shared in more left biased communities than right, it is predicted as a left biased article and vice versa. Then we maximize the similarity between news articles and predicted labels. We only make prediction about news articles which are shared in at least $2$ communities with a hope to minimize incorrect predictions. So, the bias of a subset of news articles are predicted at each step and we only update the predictions in previous E steps.
%\end{itemize}{}

% \paragraph{Inference: } Now, given that the bias nodes and all the other nodes are embedded, we can infer about the bias of any node using the following formula. Given, a node $a$ and bias $b$, the predicted bias of the node $a$ is,
% \begin{align*}
%     \operatorname{Bias}_{a}=\operatorname{arg\,max}_{b\in B} sim(a, b)
% \end{align*}
% Note that, we can identify the bias of news articles, sharing users and community centroids using the above inference rule. 

\textbf{Stopping Criterion: }At each iteration, after \textit{Step 2}, we check for the stopping criterion. We look at the predicted labels of all news articles, and if in two consecutive iterations the change in predicted labels is less than a threshold $t_{p}$, we stop.% our learning and output the communities. 
%@Shamik: what was the stopping criterion?


==> 5.1Exp.tex <==
%\begin{table*}[ht]
%\centering
%\begin{tabular}{|>{\arraybackslash}m{4.5cm}|>{\arraybackslash}m{4.5cm}|>{\arraybackslash}m{4.5cm}|}
%\hline
%\textbf{Immigration} & \textbf{Abortion} & \textbf{Gun Control}\\ \hline
%Salary Stagnation, Increase the Wage, Wage Economy, High Wage, Wage Inequality, Cheap Labor Availability, Housing Cost Increase, Tax Burden, Wealth Gap, Tax Revenue, White Nationalism, Person of Color, Born Identity, Amnesty, Asylum, Refugee, Dream Act, Family Separation Policy, DACA, Deportation of Illegal Immigrants, Deportation in General, Detention, Border Protection Wall & 
%Reproduction Right, Right of Human Life, Partial Birth Abortion, Right To Privacy, Stem Cell Research, Late Term Abortion, Selling of Fetal Tissue, Sexual Assault Victim Women, Birth Control, Women Health, Killing of Unborn Babies, Sanctity of Life, Anti-Morality of Abortion, Religious Domination on Women, Planned Parenthood, Pregnancy Centers &
%Second Amendment, Disarming of Law Abiding Citizens, Gun Import, Concealed Carry Reciprocity Act, Firearm Training Course, Gun Control for Restraining Violence, Illegal Gun, Gun Show Loophole, Gun Violence Criminal, Background Check, Universal Background Check, Terrorist Attack, Mental Health, Assault Weapon, Sports and Hunting, God Given Right of Self-Defense, Stop Gun Crime\\
%Immigration & 4,238 (L:, R:) & 4,278 (L:, R:) & 8,516 (L:, R:) & 10,374\\
%Abortion & 2,116 (L:, R: ) & 4,360 (L:, R: ) & 6,476 (L:, R: ) & 4,094\\
%Gun Control & 2,243 (L:, R: ) & 4,410 (L:, R: ) & 6,653 (L:, R: ) & 3,257\\
%\hline
%\end{tabular}
%\caption{\label{table2} Subframes identified by topic.}
%\end{table*}

\subsection{Community Evaluation Measures}
\paragraph{Identification and Evaluation of Communities}
%community assignments  - during evaluation, only users are assigned to communities based on similarity (to the community they are closest to in the embedding space). this is a hard clustering. (no fractional membership). Then we look at the documents they share and politicians they follow and add them to the community (again hard assignment) %%Motivate - multiple memberships are possible..

%Explain the implication of using an embedding space - ranking of content/label based on centroid. 
We identify communities of Twitter users and analyze the linguistic and social network behaviour of these communities. In order to validate the emerging communities, we show that they exhibit homogeneity of  relationships and linguistic content. We associate with these users other nodes they are connected to in the graph, such as the political users, documents and frames and sub-frames contained in them.

% we can think the communities as information echo-chambers who are homogeneous in social and linguistic interest. In our graph, once we know the communities of Twitter users, we can analyze their sharing behaviour, following behaviour and content interest. 

% For that in the communities of Twitter users we add the politicians followed by them, the news articles shared by them, the subframes contained in the news articles, frames contained in news articles and consider all of these entities as nodes. A Twitter user is connected to the news articles he shares and Politicians he follows.

%We consider the $15$ media frames as nodes. A news article is connected to the $3$ most frequent frames in the  article. Note that each paragraph is associated with the top $2$ frames, however we take only the top frame for each paragraph in this analysis. If any n-gram phrase from a specific subframe is used in an article, we connect that article to the subframe. Now, we define the following measures to analyze properties of each community.

\paragraph{Ranking Communities' Political Affiliation: } We can rank the communities in left-right spectrum based on the relative similarity score of their centroid embeddings with the embedding of the left ideology node in the embedding space. We take the cosine similarity measure as a similarity scoring function. In ideal case a left community will have a similarity score of $1$ and a right community will have a similarity score of $-1$, and values between the two extremes, capture communities with a more centrist perspective.

% \paragraph{Evaluating Homogeneity of Following and Sharing Behaviour Inside Community: }
\paragraph{Evaluating in-Community Behavioural Homogeneity}
To analyze the degree of homogeneity of the communities in their sharing and following behaviour we measure the use the purity measure, often used to evaluate clusters. We measure the label purity of the politicians followed-by and news articles shared-by, members of the community. The purity of a node $n^{t}$ of type $t$ is defined as follows. 
\begin{align*}
    \operatorname{Purity(n^{t})}=\frac{1}{N^{t}}\sum_{i=1}^{k}\operatorname{max}_{j}|c_{i} \cap l_{j}|
\end{align*}
Here, $N^{t}$ is total number of assignments of nodes of type $t$ in all communities, $c_{i}$ is a community out of $k$ communities and $l_{j}$ is the most common label of node type $t$ in community $c_{i}$.

 % \paragraph{Relative Importance of Nodes Inside Communities: } 
\paragraph{Relative in-Community Node Importance} 
We can define the importance of any node in a community based on the similarity score of the community centroid embedding and the node embedding learned by our model. We use cosine similarity as similarity measure. For politicians and news articles inside a community we can rank them based on this similarity score (higher score implies higher rank). For subframes we can take the average cosine similarity of the ngrams consisting a subframe. In case of frames which are not directly embedded, we can take the top $3$ most frequent frames appearing in a news article. Note that each paragraph is associated with the top $2$ frames, however, we take only the top frame for each paragraph in this analysis. After extracting the top $3$ most frequent frames in each news article, we can define the importance score of a frame $f_{k}$ in the community with centroid $c_{j}$ as follow. Here, $N_{f_{k}}^{c_{j}}$ is the number of times frame $f_{k}$ appears in community $c_{j}$ and $a_{i}$ is a news article shared in the community which contains frame $f_{k}$.
\begin{align*}
    \operatorname{Importance\_Score(f_{k})}=\frac{1}{N_{f_{k}}^{c_{j}}}\sum_{a_{i} \in c_{j}} \operatorname{sim}(a_{i}, c_{i})
\end{align*}

%To analyze the importance of a certain node in a community, we use the PageRank score \cite{page1999pagerank} which score a node in a graph based on the quality of its incoming edges. In our setting, the PageRank is a measure for analyzing homophily, as incoming edges capture shared interest, or repeating behavior, by many community members.

% importance of nodes in a homophil community where more incoming edges means the community is more interested in that particular node or the particular node is more central in the community.
Note that we can get a separate ranking for each node type (e.g., politicians, subframes, etc.) in a community based on the similarity scores as stated above.%, in most important to least important spectrum. 
After ranking the nodes of kind $t$ we normalize the rank score of a node $n^{t}_{i}$ as follows.
\begin{align*}
    \operatorname{Rank\_Score(n^{t}_{i})}=(N^{t}-r_{i}+1)/N^{t}
\end{align*}
Here, $N^{t}$ is the number of $t$-typed nodes and $r_{i}$ is the ranking of node $n^{t}_{i}$ among nodes of type $t$ inside a community. We assign $\operatorname{Rank\_Score(n^{t}_{i})}$ to $0$ if the node is not present in the community.% not ranked i.e.

% \paragraph{Relative Importance of Nodes Over Communities: } 
\paragraph{Comparing Communities based on Node Importance} 
Now to compare how the importance of nodes vary across communities, we use the Spearman's rank correlation coefficient \cite{zar2005spearman} of the ranking which measures the similarity between two sets of ranking where coefficient value of $+1$ means a perfectly positive correlation and $-1$ means a perfectly negative correlation. We can compare the importance of each type of nodes in two communities by this measure.


\subsection{Community Evaluation}
We compare our identified communities with two text clustering approach- (1) LDA \cite{blei2003latent} based topic modelling over the unigrams, bigrams and trigrams identified in the news articles, (2) BERT Embedding \cite{devlin2018bert} based article clustering. We take the pretrained BERT (base) embeddings (average of second to last layer) of each news article (truncated to $512$ tokens) and cluster them using GMM.\\%embeddings of the news articles using GMM.\\ 
To determine the number of clusters we look at the knee point of coherence score \cite{roder2015exploring} in case of LDA and BIC score in case of BERT embeddings and take the number of topics at the knee point. We assign a document to a community if the probability of the document to fall in that community is at least $1/K$, where $K$ is the number of communities found. After clustering the news articles we populate communities around them consisting of sharing users of those news articles and politicians followed by the sharing users. Note that only shared news articles on Twitter are used in the baselines as we don't know the true community assignments of the unshared news articles.\\
The purity of follow and sharing behaviour of the identified communities identified by the textual clustering baselines and our proposed approach are shown in Table \ref{tab:purity}. It can be seen that the communities formed by using only linguistic properties are outperformed by the community formed by using linguistic and social properties. Now, to observe the homophily in share, follow behaviour and subframe, frame usage we compare the ranking of politicians, news articles, subframes, frames inside each community with the leftmost and rightmost communities (according to the community rank we defined). The change in correlation of ranking by community ranking are shown in Figure \ref{fig:corr} for the three topics\footnote{We found two communities in "Gun Control" Topic which showed extremely low frequency in their sharing and following behaviour compared to the other communities found. They share $14$ news articles, follow $51.5$ politicians on average while the other communities share $470.18$ news articles and follow $342.27$ politicians on average. So, we exclude them from the correlation graphs as outliers.}. We can see from the graphs that, the correlation of ranking of politicians, news articles, subframes and frames decrease as we go from leftmost community to righmost community. That means communities are polarized in their follow, share behaviours and in the way they frame a topic. We can see from the figures that, the decrease of correlation in subframe rank is higher than the decrease of correlation in frame ranking which supports our claim that frame usage cannot strongly represent political polarization.     


%Now, we can analyze the centrality or importance of Political users, news articles, frames and subframes inside each community using PageRank score. So we rank all the nodes in each community based on their PageRank score.\\
%Now, we can rank the communities based on the relative similarity score of their centroid embeddings with the embedding of the left node in the embedding space. In ideal case a left community will have a similarity score of $1$ and a right community will have a similarity score of $0$. Now, we can analyze the community ranking in four dimensions- their follow behaviour, their news article sharing behaviour, their interest in subframes, their interest in frames. For this evaluation, for each community, we take the most important $500$ news articles shared, most important $100$ politicians followed, ranking of frames and subframes based on their importance in the community. The distributions are showed in Figure \ref{fig2}. We can see from this figure that there is a positive correlation between percentage of biased politicians followed and the rank of the community. The percentage of left politicians followed by the communities decreases as we go from extreme left bias community to the extreme right biased community. The same trend is seen in case of percentage of left biased news articles shared. So, the communities we found are polarized in their sharing and following behaviour. Now to compare the linguistic similarity among the communities, we take Spearman's Rank Correlation Coefficient of the ranking of frames and subframes in each community with the ranking in the leftmost and rightmost communities. The correlation quantifies how the importance of frames and subframes vary in communities. We can see from the figure that the correlation decays as we move from the left to right and vice versa in both cases of frames and subframes. That means the importance of frames and subframes vary by community. Also, we can see from the figures that the variance of frame ranking is low compared to the variance of subframe ranking. That proves our claim that communities are more polarized in usage of subframes than in the usage of high level frames. This proves the content homophily inside the communities. 

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.30\textwidth}
     \includegraphics[width=\textwidth]{Figures/abortion_polarization_subframe.pdf}
     \caption{Abortion}
    \end{subfigure}\par\medskip
    \begin{subfigure}[b]{0.30\textwidth}
     \includegraphics[width=\textwidth]{Figures/gun_polarization_subframe.pdf}
     \caption{Gun Control}
    \end{subfigure}\par\medskip
    \begin{subfigure}[b]{0.30\textwidth}
     \includegraphics[width=\textwidth]{Figures/immigration_polarization_subframe.pdf}
     \caption{Immigration}
    \end{subfigure}
    \caption{Polarization of Subframes.}
    \label{fig:subframe-polarity}
\end{figure}

 
\begin{figure}[ht]
  %\centering
  \begin{subfigure}{\linewidth}
  \centering
  %\includegraphics[width=.48\linewidth]{Figures/abortion_followee_distribution.pdf}
  %\includegraphics[width=.48\linewidth]{Figures/abortion_article_distribution.pdf}\\
  \includegraphics[width=.48\linewidth]{Figures/abortion_followee_rank_corr.pdf}
  \includegraphics[width=.48\linewidth]{Figures/abortion_article_rank_corr.pdf}\\
  \includegraphics[width=.48\linewidth]{Figures/abortion_subframes.pdf}
  \includegraphics[width=.48\linewidth]{Figures/abortion_frames.pdf}\\
  \caption{Abortion}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.48\linewidth]{Figures/gun_followee_rank_corr.pdf}
  \includegraphics[width=.48\linewidth]{Figures/gun_article_rank_corr.pdf}\\
  \includegraphics[width=.48\linewidth]{Figures/gun_subframes.pdf}
  \includegraphics[width=.48\linewidth]{Figures/gun_frames.pdf}
  \caption{Gun Control}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.48\linewidth]{Figures/immigration_followee_rank_corr.pdf}
  \includegraphics[width=.48\linewidth]{Figures/immigration_article_rank_corr.pdf}\\
  \includegraphics[width=.48\linewidth]{Figures/immigration_subframes.pdf}
  \includegraphics[width=.48\linewidth]{Figures/immigration_frames.pdf}
  \caption{Immigration}
  \end{subfigure}
  \caption{%The top 2 subfigures show the label distribution of followed politicians and shared articles over community ranking. 
  Each subfigure shows Spearman's rank correlation coefficient of the ranking of four types of properties inside a community with the rank of the leftmost and rightmost community for each topic. The correlation distribution is shown over community polarity ranking. Upper left graph of each subfigure shows correlation of politicians' ranks, upper right shows correlation of article ranks, lower left shows correlation of subframe ranks and lower right shows correlation of frame ranks. Communities in the blue (left) regions are identified as left communities and in the red (right) regions are identified as right communities.}
  \label{fig:corr}
\end{figure}
 
\subsubsection{Community Evaluation: }
Given the assignment of Twitter users in communities using our approach, we run some sanity checks to prove the trustworthiness of the community assignment.

\subsubsection{Polarity of Associated Properties with Communities} 
We can analyze the polarity of subframes and politicians observed in the communities and crosscheck the results to validate the community assignment. 
\paragraph{Subframe} We can analyze the polarity of the subframes by plotting their average ranking score in the left biased communities vs their average ranking score in right biased communities. The plots are shown in Figure \ref{fig:subframe-polarity}. We can see that in the topic \textit{Abortion}, stance points which are opposing abortion have higher ranking in the right communities, where in the left communities stance points related to women rights and freedom are more highly ranked. The trend is consistent with Republican and Democrat stances in the issue \textit{Abortion}. Note that, "Women health" issue is ranked highest in both type of communities which means it is broader than a polarized stance and discussed in both type of communities. The polarization graph for other two topics are attached in the Appendix section because of space constraint.

%\paragraph{Hashtag} Hashtags are popularly used as topic indicator in Tweets. But in profile description Twitter users use hashtags which is more related to his overall political bias. So, we define a hashtag classification task to inversely validate the community assignment of Twitter users. For that we extract all the hashtags from the user description section of all the Twitter users in our graph and human annotate the hashtags as \textit{Left} or \textit{Right} biased. Note that we only take the hashtags which have political meaning and high bias. We found $207,154,346$ unique hashtags in the topics \textit{Abortion, Gun Control and Immigration} respectively. Then we can include the hashtags in the communities the same way we included the subframes, frames, politicians and news articles and rank them using PageRank score. Then we classify a hashtag as left if it has a higher average ranking score in left biased communities and right if vice versa. Following this procedure we get a macro F1 score of $98.06\%,95.45\%,95.66\%$ in the hashtag classification task in the topics \textit{Abortion, Gun Control and Immigration} respectively which proves the validdity of our community assignments.

% \paragraph{Politicians} Similar to subframes, we can rank politicians based on their importance in left and right communities. We compare the Spearman's rank correlation coefficient between this ranking, averaged in left and right communities separately, and the politicians' ideology scores assigned by GovTrack\footnote{https://www.govtrack.us}, ranking them from most conservative to most liberal, based on their voting records.  Results shown in Figure \ref{fig:politician-rank} validate the learned political representation of communities, as the GovTrack ranking negatively correlates with left-leaning communities and positively with right-winged. 

% \begin{figure}[ht]
% \begin{center}
% \includegraphics[width=0.4\textwidth]{Figures/combined_gt_followee_rank_corr.pdf}
% \caption{Rank Corr. with GovTrack Rank. of Politicians}
% \label{fig:politician-rank}
% \end{center}
% \end{figure}


% We can identify the most popular politicians in both left and right communities similarly as subframes and hashtags using their ranking scores. Then we get two rankings (from most popular to least popular) of politicians in left communities and right communities based on their average ranking score in left and right communities respectively. We can form a ground truth ranking (from most conservative to most liberal) of politicians from the ideology scores assigned to them by GovTrack\footnote{https://www.govtrack.us}. Then we can compare the Spearman's rank correlation coefficient of the ranking of the politicians in the left and right communities with the ground truth ranking. We could find GovTrak score for $411$ politicians out of $578$ politicians in our graph. So, we compare the rankings of these $411$ politicians. The results are shown in Table \ref{tab:politician-corr}. We can see that, the popularity rank of the politicians in the left communities has a negative correlation with the ground truth ranking of most conservative to most liberal and, the rank of the politicians in the right communities has a positive correlation with the ground truth ranking which validates our community assignment.

%\begin{table}[ht]
%\centering
%\scalebox{0.82}{
%\begin{tabular}{>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{2.5cm}|>{\centering\arraybackslash}m{2.5cm}}
%\hline
%Corr. of Ground Truth Rank & With Rank in Right (Ideal +1) & With Rank in Left (Ideal -1)\\ %\hline\hline
%\textbf{Abortion} & 0.549 & -0.619  \\
%\textbf{Gun Control} & 0.433 & -0.620 \\
%\textbf{Immigration} & 0.376 & -0.669 \\
%\hline
%\end{tabular}}
%\caption{\label{table2} Corr. between ideology scores and politicians importance ranking in left and right communities.}
%\label{tab:politician-corr}
%\end{table}


\subsection{Bias Detection Task in News Articles} Now to validate the learned embeddings and for analyzing the effect of the community embeddings we define a text classification task over the learned embeddings of the news articles. We identify the bias of news articles by the inference formula defined in Modeling section. The results are shown in Table \ref{tab:text-classification}. The Label Propagation approach in the table infers the bias of the news articles after learning the embeddings only using the known initial objectives. The EM approach in the table infers labels after performing EM steps but without article to ngram objectives. We can see from the table that, in all of the three datasets EM with community objectives outperforms the label propagation step. Also, we can see a large improvement in case of the unshared news articles when we connect them to the graph via "Article to Ngram" objective which validates our claim of biased phrases. Note that when there is no "Article to Ngram" objective, we still can get the embeddings of the unshared news articles from the trained text encoder and predict the label of then using the same inference rule. We show the results of fully supervised classification results of the news articles using HLSTM and BERT (base) embeddings. Note that BERT classification results are worse than HLSTM as the news articles are truncated to $512$ tokens and more than $50\%$ news articles in each topic have more than $512$ tokens.      
\paragraph{Qualitative Analysis of Document Assignment to Communities } We select $6$ news articles (Table \ref{tab:hitmap}) from the unshared news article set in Abortion topic and compare plot a hitmap to see the correlation between the community ranking and cosine similarity of the articles with the centroids of the communities and found the heatmap shown in Figure \ref{fig:hitmap}. We can see that the articles are closer to the communities according to their bias and the subframe interest of the communities, although they were not included in the communities during embedding learning. This evaluation proves the usefulness of the communities and indicates a way to recommend unshared news articles to the identified communities correctly according to their interest. 

\begin{table}[ht]
\begin{center}
\scalebox{0.75}{
\begin{tabular}{>{\arraybackslash}m{5.6cm}|>{\arraybackslash}m{3.6cm}}
\hline
ID-Headline (Bias) & Subframes Used (Community ranks)\\
\hline
a1-Activists see threat to Roe precedent (L) & Right To Privacy (4) \\
\hline
a2-U.S. Court Rejects Alabama Abortion Restrictions, Cites Harassment Providers Face (L) & Reprod. Right (1, 3), Birth Control (1, 3)\\
\hline
a3-Warren Is Worth the Headache (L) & Religious Dom. (2, 5)\\
\hline
a4-Why Even Pro-Choice Americans Should be Upset with Planned Parenthood (R) &  Sel. of Fet. Tiss. (6, 7), Sex. Assult Vict. Wom. (-), Wom. Health (-)\\
\hline
a5-Abusive Abortion Activists Terrorize Children at Pro-Life Rally (R) & Right of Hum. Life (-)\\
\hline
a6-A Game Changer for the Abortion Debate (R) & Right of Hum. Life (-), Sanct. of Life (8, 10), \\
\hline
\end{tabular}}
\caption{Selected News Articles for Evaluation. Each subframe is associated with ranked communities in which they appear in top-2 most important subframes.}
\label{tab:hitmap}
\end{center}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{Figures/abortion_article_corr.pdf}
\caption{Heatmap}
\label{fig:hitmap}
\end{figure}

%\begin{figure*}[h]
%    \centering
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/abortion_followee_rank_corr.pdf}
%     \caption{}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/abortion_article_rank_corr.pdf}
%     \caption{}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/abortion_subframes.pdf}
%     \caption{}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/abortion_frames.pdf}
%     \caption{}
%    \end{subfigure}\\
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/gun_followee_rank_corr.pdf}
%     \caption{}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/gun_article_rank_corr.pdf}
%     \caption{}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/gun_subframes.pdf}
%     \caption{}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/gun_frames.pdf}
%     \caption{}
%    \end{subfigure}\\
%    \begin{subfigure}[b]{0.215\textwidth}
%     \includegraphics[width=\textwidth]{Figures/immigration_followee_distribution.pdf}
%     \caption{}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/immigration_article_distribution.pdf}
%     \caption{}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/immigration_subframes.pdf}
%     \caption{}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{Figures/immigration_frames.pdf}
%     \caption{}
%    \end{subfigure}
%    
%    \caption{Figure (a)-(d) describes properties of the communities found in topic Abortion, Figure (e)-(h) for Gun Control and Figure (i)-(l) for Immigration. The 1st column of figures (Figure (a), (e), (i)) describe the distribution of \% of labeled politicians followed by the communities, 2nd column of figures (Figure (b), (f), (j)) describe the distribution of \% of labeled news articles shared by the communities, 3rd column of figures (Figure (c), (g), (k)) show the change in Spearman's rank correlation of subframe ranking in the communities with the leftmost and rightmost communities, 4th column of figures (Figure (d), (h), (l)) show the change in Spearman's rank correlation of frame ranking in the communities with the leftmost and rightmost communities. All of the distributions are over community ranking. Communities in the blue (left) region are annotated as left communities and in the red (right) region are annotated as right communities.}
%    \label{fig2}
%\end{figure*}

%Given we have identified the polarized communities and have seen a strong correlation between the subframe usage and community bias, now, we can analyze the polarity of the subframes based on our discovered communities and their bias. For this we trust the identified label of each community by our model and measure the average ranking score of each subframe in left and right biased communities. Most important subframe in a community is given the highest ranking score. We ploting these two ranking scores in X and Y axes, we can see the polarity of each subframe in Figure \ref{fig4}. \textcolor{red}{Need to add reference to validate the polarization of subframes.}








% %%%%%%%%%%%%%%subframespol
% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[b]{0.30\textwidth}
%      \includegraphics[width=\textwidth]{Figures/abortion_polarization_subframe.pdf}
%      \caption{Abortion}
%     \end{subfigure}\par\medskip
%     \begin{subfigure}[b]{0.30\textwidth}
%      \includegraphics[width=\textwidth]{Figures/gun_polarization_subframe.pdf}
%      \caption{Gun Control}
%     \end{subfigure}\par\medskip
%     \begin{subfigure}[b]{0.30\textwidth}
%      \includegraphics[width=\textwidth]{Figures/immigration_polarization_subframe.pdf}
%      \caption{Immigration}
%     \end{subfigure}
%     \caption{Polarization of Subframes}
%     \label{fig:subframe-polarity}
% \end{figure}

 
 
% \begin{table*}[h]
% \begin{center}
%  \scalebox{0.71}{\begin{tabular}{>{\arraybackslash}m{3.6cm}||>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.7cm}||>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.7cm}||>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.7cm}} 
%  \hline 
% \textsc{Model} & \multicolumn{3}{c}{\textsc{\textbf{Abortion}}} & \multicolumn{3}{c}{\textsc{\textbf{Gun Control}}} & \multicolumn{3}{c}{\textsc{\textbf{Immigration}}}\\ [0.5ex]
% \cline{2-10}
% &   \textsc{\# Comm.}   &   \textsc{P(Share)}   &   \textsc{P(Follow)}   &   \textsc{\# Comm.} &   \textsc{P(Share)}   &   \textsc{P(Follow)}   &   \textsc{\# Comm.}   &   \textsc{P(Share)} &   \textsc{P(Follow)}\\
%  \hline
%  LDA   & 7  & 0.59  & 0.53 & 9  & 0.61  & 0.53 & 17 & 0.59  & 0.53 \\
%  \hline
%  Bert  & 9  & 0.65  & 0.53  & 13  & 0.66  & 0.54  & 20  & 0.74 & 0.53 \\
%  \hline
%  Label Propagation  & 4 & 0.82 & 0.55 & 10 & \textbf{0.83} & 0.61 & 10 & 0.84 & 0.60 \\
%  \hline
%  EM                 & 9 & \textbf{0.89} & 0.60 & 10 & \textbf{0.83} & 0.62 & 12 & 0.85 & 0.63 \\
%  \hline
%  EM+Ngram Objective & 11 & \textbf{0.89} & \textbf{0.63} & 13 & 0.82 & \textbf{0.66} & 18 & \textbf{0.87} & \textbf{0.67} \\
%  \hline
%  \end{tabular}}
% \caption{Comparison of Purity of following and sharing behaviour of communities found by different embeddings approaches. The function P() defines the purity.}
% \label{tab3}
% \end{center}
% \end{table*}




\begin{figure}[ht]
  %\centering
  \begin{subfigure}{\linewidth}
  \centering
  %\includegraphics[width=.48\linewidth]{Figures/abortion_followee_distribution.pdf}
  %\includegraphics[width=.48\linewidth]{Figures/abortion_article_distribution.pdf}\\
  \includegraphics[width=.48\linewidth]{Figures/abortion_followee_rank_corr.pdf}
  \includegraphics[width=.48\linewidth]{Figures/abortion_article_rank_corr.pdf}\\
  \includegraphics[width=.48\linewidth]{Figures/abortion_subframes.pdf}
  \includegraphics[width=.48\linewidth]{Figures/abortion_frames.pdf}\\
  \caption{Abortion}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.48\linewidth]{Figures/gun_followee_rank_corr.pdf}
  \includegraphics[width=.48\linewidth]{Figures/gun_article_rank_corr.pdf}\\
  \includegraphics[width=.48\linewidth]{Figures/gun_subframes.pdf}
  \includegraphics[width=.48\linewidth]{Figures/gun_frames.pdf}
  \caption{Gun Control}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.48\linewidth]{Figures/immigration_followee_rank_corr.pdf}
  \includegraphics[width=.48\linewidth]{Figures/immigration_article_rank_corr.pdf}\\
  \includegraphics[width=.48\linewidth]{Figures/immigration_subframes.pdf}
  \includegraphics[width=.48\linewidth]{Figures/immigration_frames.pdf}
  \caption{Immigration}
  \end{subfigure}
  \caption{%The top 2 subfigures show the label distribution of followed politicians and shared articles over community ranking. 
  Each subfigure shows Spearman's rank correlation coefficient of the ranking of four types of properties inside a community with the rank of the leftmost and rightmost community for each topic. The correlation distribution is shown over community polarity ranking. Upper left graph of each subfigure shows correlation of politicians' ranks, upper right shows correlation of article ranks, lower left shows correlation of subframe ranks and lower right shows correlation of frame ranks. Communities in the blue (left) regions are identified as left communities and in the red (right) regions are identified as right communities.}
  \label{fig:corr}
\end{figure}





\begin{figure}[ht]
  %\centering
  \begin{subfigure}{\linewidth}
  \centering
  %\includegraphics[width=.48\linewidth]{Figures/abortion_followee_distribution.pdf}
  %\includegraphics[width=.48\linewidth]{Figures/abortion_article_distribution.pdf}\\
  \includegraphics[width=.489\linewidth]{Figures/abortion_followee_rank_corr.pdf}
  \includegraphics[width=.489\linewidth]{Figures/abortion_article_rank_corr.pdf}\\
  \caption{Abortion}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.489\linewidth]{Figures/gun_followee_rank_corr.pdf}
  \includegraphics[width=.489\linewidth]{Figures/gun_article_rank_corr.pdf}\\
  \caption{Gun Control}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.489\linewidth]{Figures/immigration_followee_rank_corr.pdf}
  \includegraphics[width=.489\linewidth]{Figures/immigration_article_rank_corr.pdf}\\
  \caption{Immigration}
  \end{subfigure}
  \caption{%The top 2 subfigures show the label distribution of followed politicians and shared articles over community ranking. 
 Spearman's rank correlation coefficient of the ranking of politicians and news article nodes inside a community with the ranking of the leftmost and rightmost community for each topic. 
%  The correlation distribution is shown over community polarity ranking. Upper left graph of each subfigure shows correlation of politicians' ranks, upper right shows correlation of article ranks, lower left shows correlation of subframe ranks and lower right shows correlation of frame ranks. 
 Communities in the blue (left) regions are identified as left communities and the vice-versa.}
  \label{fig:socialCor}
\end{figure}



\begin{figure}[ht]
  %\centering
  \begin{subfigure}{\linewidth}
  \centering
  %\includegraphics[width=.48\linewidth]{Figures/abortion_followee_distribution.pdf}
  %\includegraphics[width=.48\linewidth]{Figures/abortion_article_distribution.pdf}\\
   \includegraphics[width=.48\linewidth]{Figures/abortion_subframes.pdf}
  \includegraphics[width=.48\linewidth]{Figures/abortion_frames.pdf}
  \caption{Abortion}
  \end{subfigure} 
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.48\linewidth]{Figures/gun_subframes.pdf}
  \includegraphics[width=.48\linewidth]{Figures/gun_frames.pdf}
  \caption{Gun Control}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.48\linewidth]{Figures/immigration_subframes.pdf}
  \includegraphics[width=.48\linewidth]{Figures/immigration_frames.pdf}
  \caption{Immigration}
  \end{subfigure}
  \caption{%The top 2 subfigures show the label distribution of followed politicians and shared articles over community ranking. 
    Spearman's rank correlation coefficient of the ranking of frames and subframes inside a community with the ranking of the leftmost and rightmost community for each topic. 
%  The correlation distribution is shown over community polarity ranking. Upper left graph of each subfigure shows correlation of politicians' ranks, upper right shows correlation of article ranks, lower left shows correlation of subframe ranks and lower right shows correlation of frame ranks. 
 %Communities in the blue (left) regions are identified as left communities and in the red (right) regions are identified as right communities.}
}
  \label{fig:corr}
\end{figure}

 

==> 5Experiments.tex <==



\begin{table*}[]
\begin{center}
 \scalebox{0.71}{\begin{tabular}{>{\arraybackslash}m{3.6cm}||>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.7cm}||>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.7cm}||>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.7cm}} 
 \hline 
\textsc{Model} & \multicolumn{3}{c}{\textsc{\textbf{Abortion}}} & \multicolumn{3}{c}{\textsc{\textbf{Gun Control}}} & \multicolumn{3}{c}{\textsc{\textbf{Immigration}}}\\ [0.5ex]
\cline{2-10}
&   \textsc{\# Comm.}   &   \textsc{P(Share)}   &   \textsc{P(Follow)}   &   \textsc{\# Comm.} &   \textsc{P(Share)}   &   \textsc{P(Follow)}   &   \textsc{\# Comm.}   &   \textsc{P(Share)} &   \textsc{P(Follow)}\\
 \hline
 LDA   & 7  & 0.59  & 0.53 & 9  & 0.61  & 0.53 & 17 & 0.59  & 0.53 \\
 \hline
 Bert  & 9  & 0.65  & 0.53  & 13  & 0.66  & 0.54  & 20  & 0.74 & 0.53 \\
 \hline
 Label Propagation  & 4 & 0.82 & 0.55 & 10 & \textbf{0.83} & 0.61 & 10 & 0.84 & 0.60 \\
 \hline
 EM                 & 9 & \textbf{0.89} & 0.60 & 10 & \textbf{0.83} & 0.62 & 12 & 0.85 & 0.63 \\
 \hline
 EM+SF Objective & 11 & \textbf{0.89} & \textbf{0.63} & 13 & 0.82 & \textbf{0.66} & 18 & \textbf{0.87} & \textbf{0.67} \\
 \hline
 \end{tabular}}
\caption{Comparison of Purity of following and sharing behaviour of communities found by different embeddings approaches. The function P() defines the purity (at most 1, higher better).}
\label{tab:purity}
\end{center}
\end{table*}


\begin{table*}[h]
    \begin{center}
    \scalebox{0.71}{\begin{tabular}{>{\arraybackslash}m{3.6cm}||>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.6cm}|>{\centering\arraybackslash}m{1.7cm}||>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.6cm}|>{\centering\arraybackslash}m{1.7cm}||>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1.6cm}|>{\centering\arraybackslash}m{1.7cm}} 
    \hline 
    \textsc{Model} & \multicolumn{3}{c}{\textsc{\textbf{Abortion}}} & \multicolumn{3}{c}{\textsc{\textbf{Gun Control}}} & \multicolumn{3}{c}{\textsc{\textbf{Immigration}}}\\ [0.5ex]
    \cline{2-10}
    &   \textsc{Shared}   &   \textsc{Unshared}   &   \textsc{Overall}   &   \textsc{Shared} &   \textsc{Unshared}   &   \textsc{Overall}   &   \textsc{Shared}   &   \textsc{Unshared} &   \textsc{Overall}\\
     \hline
     Label Propagation  & 88.18 & 69.05 & 75.47 & 81.67 & 55.05 & 64.00 & 87.16 & 47.52 & 67.87 \\
     \hline
     EM                 & \textbf{90.20} & 68.21 & 75.41 & 83.11 & 54.47 & 64.19 & 91.63 & 45.53 & 68.88 \\
     \hline
     EM+SF Objective & 89.71 & \textbf{73.55} & \textbf{79.23} & \textbf{84.62} & \textbf{60.63} & \textbf{68.79} & \textbf{92.94} & \textbf{68.65} & \textbf{81.51} \\
     \hline
     \hline
     HLSTM (3 fold CV)  & ---  & ---  & 79.84 (1.0) & ---  & ---  & 75.18 (1.8)  & ---  & --- & 85.57 (0.3)\\
     \hline
     BERT (3 fold CV)   & ---  & ---  & 81.58 (1.8) & ---  & ---  & 73.21 (0.7) & ---  & --- & 79.72 (3.7)\\
     \hline
 \end{tabular}}
\caption{The first three rows show the text classification results for distant supervision settings. The last two rows are \textit{supervised} classification results with standard deviation. We report macro F1 scores.}
\label{tab:text-classification}
\end{center}
\end{table*}


\section{Experiments}\label{sec:experiments}
Our experimental settings are designed to evaluate our community embedding ability to characterize polarization in news media on several controversial issues. We conduct this analysis at the \textit{community level}, by validating the community structure emerging from the data using several measures and analyzing the characteristics of each community. We also conduct \textit{document level} analysis, showing that our approach captures political perspective in individual documents, a useful result on its own right. We begin with our experimental settings and several measures used for evaluating the embedding space, and then describe our results.

\paragraph{Experimental Settings} We run our proposed model for identifying communities in the three topics. For \textit{Abortion, Gun Control and Immigration} we run the embeddings learning for $30, 30, 50$ epochs respectively in \textit{Step 1} described in Section \ref{sec:detected-relations}. While determining the number of communities in \textit{Step 2} we set threshold $t_{n}$ as $1, 10, 1$ in case of \textit{Abortion, Gun Control and Immigration} respectively. We assign a Twitter user node to a community if it has a probability of at least $50\%$ to fall under that community\footnote{We experimented with lower thresholds of probability to encourage assignment of one user to multiple communities and it was seen that community assignment does not change.}. For stopping criteria, we set the threshold $t_{p}$ to ($10\%$ for Immigration, $5\%$ for Gun control and Abortion) and ($15\%$ for Immigration, $10\%$ for Gun control and Abortion) when learning without and with the  sub-frame objectives respectively. Note that the sub-frame expressions objective, connects unshared news articles to the network via the similarity in expression used, resulting in a larger training set and we use a larger threshold for stopping. We truncate each news article to $20$ sentences before passing through the HLSTM encoder. The single layer HLSTM encoder takes $300$-d Glove word embeddings as inputs and maps to a $300$-d hidden layer. Embeddings of all of the other nodes were randomly initialized in $300$-d space. $\lambda_{r}$ in Section \ref{sec:observed-relations} is set to $2$ for the \textit{article} to \textit{sub-frame} objective and $1$ for all others.     

\subsection{Community Evaluation Measures}
%  \paragraph{Identification and Evaluation of Communities}     \includegraphics[width=0.9\textwidth]{Figures/immigration_polarization_subframe.pdf}


 We identify user communities and analyze the linguistic and social behaviour of these communities. In order to validate the emerging communities, we show that they exhibit homogeneity in relationships and linguistic content. To do that, we look at different properties captured by the embedding space, consisting of community embedding (i.e., their mean vector $\Psi$), as well as articles, users, sub-frames expressions and political labels.
 
%  We associate with these users other nodes they are connected to in the graph, such as the political users, documents and frames and sub-frames contained in them.

% we can think the communities as information echo-chambers who are homogeneous in social and linguistic interest. In our graph, once we know the communities of Twitter users, we can analyze their sharing behaviour, following behaviour and content interest. 

% For that in the communities of Twitter users we add the politicians followed by them, the news articles shared by them, the subframes contained in the news articles, frames contained in news articles and consider all of these entities as nodes. A Twitter user is connected to the news articles he shares and Politicians he follows.

%We consider the $15$ media frames as nodes. A news article is connected to the $3$ most frequent frames in the  article. Note that each paragraph is associated with the top $2$ frames, however we take only the top frame for each paragraph in this analysis. If any n-gram phrase from a specific subframe is used in an article, we connect that article to the subframe. Now, we define the following measures to analyze properties of each community.

\vspace{1pt}\noindent\textbf{(1) Ranking Communities' Political Affiliation: } We can rank the communities in left-right spectrum based on the relative cosine similarity score of their centroid embeddings with the embedding of the left ideology node in the embedding space. Based on this score, we place communities on a continuous spectrum between 1 (left) and -1 (right). 

% We take the cosine similarity measure as a similarity scoring function. In ideal case a left community will have a similarity score of $1$ and a right community will have a similarity score of $-1$, and values between the two extremes, capture communities with a more centrist perspective.

% \paragraph{Evaluating Homogeneity of Following and Sharing Behaviour Inside Community: }
\vspace{2pt}
\noindent\textbf{(2) Evaluating in-Community Homogeneity:}
\vspace{1pt}
To analyze the degree of homogeneity of communities we use the purity measure, often used to evaluate clusters. We measure the label purity of the politicians followed-by and news articles shared-by, members of the community. The purity of a node $n^{t}$ of type $t$ is defined as follows. 
{\footnotesize
\vspace{-2pt}
\begin{align*}
    \operatorname{Purity(n^{t})}=\frac{1}{N^{t}}\sum_{i=1}^{k}\operatorname{max}_{j}|c_{i} \cap l_{j}|
\end{align*}
    \vspace{-2pt}
}
$N^{t}$ is total number of nodes of type $t$ in all communities, $c_{i}$ is a community and $l_{j}$ is the most common label for node type $t$ in community $c_{i}$.

 % \paragraph{Relative Importance of Nodes Inside Communities: } 
\vspace{1pt}\noindent\textbf{(3) Relative in-Community Node Importance} Another way to evaluate properties of communities is by ranking the nodes associated with the community. Using the similarity between the community centroid and a given node embedding is a natural ranking score, used for ranking politicians and news articles. We score sub-frames by averaging the similarity scores between the embedding of the sub-frame's expressions and the community centroid.
% We can define the importance of any node in a community based on the similarity score of the community centroid embedding and the node embedding learned by our model. We use cosine similarity as similarity measure. For politicians and news articles inside a community we can rank them based on this similarity score (higher score implies higher rank). For subframes we can take the average cosine similarity of the ngrams consisting a subframe.
In case of frames, which are not directly embedded, we extract the 3 most frequent frames appearing in each article,
% we can take the top $3$ most frequent frames appearing in a news article. Note that each paragraph is associated with the top $2$ frames, however, we take only the top frame for each paragraph in this analysis. After extracting the top $3$ most frequent frames in each news article, 
and define the importance score of a frame $f_{k}$ w.r.t a community $c_{j}$ as follows:
{\small
\begin{align*}
    \operatorname{Score(f_{k},c_j)}=\frac{1}{N_{f_{k}}^{c_{j}}}\sum_{a_{i} \in c_{j}} \operatorname{sim}(a_{i}, c_{j})
\end{align*}}
Here, $N_{f_{k}}^{c_{j}}$ is the number of times frame $f_{k}$ appears in community $c_{j}$ and $a_{i}$ is a news article shared in the community which contains frame $f_{k}$.

%To analyze the importance of a certain node in a community, we use the PageRank score \cite{page1999pagerank} which score a node in a graph based on the quality of its incoming edges. In our setting, the PageRank is a measure for analyzing homophily, as incoming edges capture shared interest, or repeating behavior, by many community members.

% importance of nodes in a homophil community where more incoming edges means the community is more interested in that particular node or the particular node is more central in the community.
% Note that we can get a separate ranking for each node type (e.g., politicians, subframes, etc.) in a community based on the similarity scores as stated above.%, in most important to least important spectrum. 
After ranking the nodes of kind $t$ we normalize the rank score of a node $n^{t}_{i}$ as follows.
{\footnotesize
\begin{align*}
    \operatorname{Rank\_Score(n^{t}_{i})}=(N^{t}-r_{i}+1)/N^{t}
\end{align*}}
Here, $N^{t}$ is the number of $t$-typed nodes and $r_{i}$ is the ranking of node $n^{t}_{i}$ among nodes of type $t$. %We assign $\operatorname{Rank\_Score(n^{t}_{i})}$ to $0$ if the node is not present in the community.% not ranked i.e.

% \paragraph{Relative Importance of Nodes Over Communities: } 
\vspace{1pt}\noindent\textbf{(4) Ranking-based Communities Comparison} 
Comparing how the importance of nodes vary across communities, we use the Spearman's rank correlation coefficient \cite{zar2005spearman} of the ranking which measures the similarity between two sets of ranking where coefficient value of $+1$ means a perfectly positive correlation and $-1$ means a perfectly negative correlation.

% We can compare the importance of each type of nodes in two communities by this measure.


\subsection{Evaluating Political Perspective}
Our first set of results aim to evaluate how political perspective is captured in the community embedding space and whether this information can help reduce uncertainty when it comes to evaluating the political perspectives expressed in news articles. 

\noindent\textbf{(1) Validating the Communities Political Representation.} To help ground our community evaluation, we use the politicians' ideology scores assigned by GovTrack\footnote{https://www.govtrack.us}, ranking them from most conservative to most liberal, based on their voting records. We use Spearman's rank correlation coefficient between this ranking and the ranking of politicians in each community (ranked based on their similarity to the community centroid, as explained above).  The results, shown in Fig. \ref{fig:politician-rank}, validate the learned political representation as the GovTrack ranking negatively correlates with left-leaning communities and positively with right-leaning.

% \paragraph{Politicians} Similar to subframes, we can rank politicians based on their importance in left and right communities. We compare the Spearman's rank correlation coefficient between this ranking, averaged in left and right communities separately, and the politicians' ideology scores assigned by GovTrack\footnote{https://www.govtrack.us}, ranking them from most conservative to most liberal, based on their voting records.  Results shown in Figure \ref{fig:politician-rank} validate the learned political representation of communities, as the GovTrack ranking negatively correlates with left-leaning communities and positively with right-winged. 

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.24\textwidth]{Figures/combined_gt_followee_rank_corr.pdf}
\vspace{-5pt}
\caption{Rank Corr. with GovTrack Ranking}
\label{fig:politician-rank}
\end{center}
\vspace{-15pt}
\end{figure}

\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.27\textwidth}
     \includegraphics[width=\textwidth]{Figures/abortion_polarization_subframe.pdf}
     \caption{Abortion}
    \end{subfigure}\medskip~~~
    \begin{subfigure}[b]{0.27\textwidth}
     \includegraphics[width=\textwidth]{Figures/gun_polarization_subframe.pdf}
     \caption{Gun Control}
    \end{subfigure}\medskip~~~
    \begin{subfigure}[b]{0.27\textwidth}
     \includegraphics[width=\textwidth]{Figures/immigration_polarization_subframe.pdf}
     \caption{Immigration}
    \end{subfigure}
    \vspace{-20pt}
    \caption{Polarization of Subframes.}
    \label{fig:subframe-polarity}
\end{figure*}


 
% \subsubsection{Community Purity}
\noindent\textbf{(2) Communities' Label Homogeneity}. We have shown above that the overall political score associated with each community matches an external data point, the ranking of politicians based on their ideology scores. Now, instead of looking at the community as a whole, we evaluate its cohesion, by measuring the degree of agreement between its members. We calculate the average purity score of communities, w.r.t. the label of the articles they share and politicians they follow. Intuitively, a higher score indicates stronger agreement between members, and a score of 0.5 corresponds to a uniform distribution of labels in each community. 

 We compared three versions of our model, the first using the  graph embedding directly for clustering, without iterating multiple times (label-propagation), and  our EM-inspired approach, without and with, adding the sub-frame expression nodes to the embedding objective (EM, EM+SF, respectively). We also compared our models with two text clustering approaches. (1) LDA \cite{blei2003latent} based topic modeling over the unigrams, bigrams and trigrams identified in the news articles, (2) Pre-trained BERT Embedding \cite{devlin2018bert} based GMM for clustering articles. To determine the number of clusters we look at the knee point of coherence score \cite{roder2015exploring} in case of LDA and BIC score in case of BERT embeddings and take the number of topics at the knee point. After clustering, we create communities by adding users sharing the news articles and politicians followed by the sharing users.
The purity results are shown in Table \ref{tab:purity}. Text-based approaches fail to capture political meaning, as social information containing this signal is not represented during clustering, resulting in low purity scores. While BERT capture political information better than LDA for articles, follow purity is close to uniform in both. Interestingly, our communities capture political information in text, resulting in highly biased communities with high article (share) purity. As we discuss later in the paper, the relatively lower follow purity stems from the fact that centrist communities tend to have low purity, as politicians from both sides are followed in these.\\
% It can be seen that the communities formed by using only linguistic properties are outperformed by the communities formed by using linguistic and social properties. 
% We compare our identified communities with two text clustering approach- (1) LDA \cite{blei2003latent} based topic modelling over the unigrams, bigrams and trigrams identified in the news articles, (2) BERT Embedding \cite{devlin2018bert} based article clustering. We take the pretrained BERT (base) embeddings (average of second to last layer) of each news article (truncated to $512$ tokens) and cluster them using GMM. To determine the number of clusters we look at the knee point of coherence score \cite{roder2015exploring} in case of LDA and BIC score in case of BERT embeddings and take the number of topics at the knee point. We assign a document to a community if the probability of the document to fall in that community is at least $1/K$, where $K$ is the number of communities found. After clustering the news articles we populate communities around them consisting of sharing users of those news articles and politicians followed by the sharing users. Note that only shared news articles on Twitter are used in the baselines as the true community assignments of the unshared articles are unknown.\\
% The purity of follow and sharing behaviour of the identified communities identified by the textual clustering baselines and our proposed approach are shown in Table \ref{tab:purity}. It can be seen that the communities formed by using only linguistic properties are outperformed by the communities formed by using linguistic and social properties. 
\noindent\textbf{(3) Bias Detection Task in News Articles.} Finally, we validate our ability to represent political information by defining a text classification task, detecting the political bias of news articles, over the learned embedding space, using the inference formula for political bias in section~\ref{sec:observed-relations}. The results are shown in Table \ref{tab:text-classification}.  We compare the three versions of our system (explained above in (2)), and two supervised systems, the first using the same text encoder as our embedding procedure (HLSTM) and the popular BERT representation (truncating the articles to the first 512 tokens). When evaluating our community embedding models, we separate between performance on \texit{shared} articles and \texit{unshared} articles, for whom no indirect social supervision is available. Despite having no direct supervision, our model performs almost comparably in most cases to supervised classifiers. Interestingly, representing the sub-frames results in a significant performance improvement for unshared documents, as they provide a bridge  connecting articles with and without social supervision, based on their contents.  

% Now to validate the learned embeddings and for analyzing the effect of the community embeddings we define a text classification task over the learned embeddings of the news articles. We identify the bias of news articles by the inference formula defined in Modeling section. The results are shown in Table \ref{tab:text-classification}. The Label Propagation approach in the table infers the bias of the news articles after learning the embeddings only using the known initial objectives. The EM approach in the table infers labels after performing EM steps but without article to ngram objectives.

% We can see from the table that, in all of the three datasets EM with community objectives outperforms the label propagation step. Also, we can see a large improvement in case of the unshared news articles when we connect them to the graph via "Article to Ngram" objective which validates our claim of biased phrases. Note that when there is no "Article to Ngram" objective, we still can get the embeddings of the unshared news articles from the trained text encoder and predict the label of then using the same inference rule. We show the results of fully supervised classification results of the news articles using HLSTM and BERT (base) embeddings. Note that BERT classification results are worse than HLSTM as the news articles are truncated to $512$ tokens and more than $50\%$ news articles in each topic have more than $512$ tokens.  



\subsection{Analyzing Frame Usage}
% \noindent\textbf{(1) Polarity of Associated Properties with Communities} 


% \noindent\textbf{(2) Qualitative Analysis of Document Assignment to Communities} 

To help provide intuition about the framing representation learned by our model, we selected 6 news articles from the unshared set of abortion articles, extracted the sub-frames appearing in each and identified the communities in which these sub-frames are top ranked. Then, we plot a heatmap capturing the cosine similarity of these documents with each one of the 11 communities detected for abortion articles, ordered from left-to-right based on their political affiliation score.
The analysis demonstrates several points: (1) it shows how political bias is captured in the embedding space. Left-winged articles \textit{a1-a3} have a high similarity score with the extreme left community (\textit{c1}) , and similarly, right-winged articles \textit{a4-a6} have a high similarity score with extreme right communities (\textit{c10,c11}). Politically affiliated communities, on either side, are never positively associated with articles expressing opposite views. (2) it also shows the topic preference of each community. As communities move towards the center, the higher ``heat'' cannot be explained by political agreement alone, in this case the sub-frame help explain the specific aspects of the abortion debate relevant for each community, by observing the match between sub-frames identified in documents and the rank of these sub-frames for each community (e.g., \textit{c3}, while left leaning, is only associated with \textit{a2}, which matches its sub-frame ranking).

% We select $6$ news articles (Table \ref{tab:hitmap}) from the unshared news article set in Abortion topic and compare plot a hitmap to see the correlation between the community ranking and cosine similarity of the articles with the centroids of the communities and found the heatmap shown in Figure \ref{fig:hitmap}.



\begin{table}[ht]
\begin{center}
\scalebox{0.69}{
\begin{tabular}{>{\arraybackslash}m{6.5cm}|>{\arraybackslash}m{4cm}}
\hline
\textbf{ID-Headline} (Bias) & \textbf{Subframes} (Com. rank)\\
\hline
a1-\textit{Activists see threat to Roe precedent} (L) & Right To Privacy (4) \\
\hline
a2-\textit{Court Rejects AL Abortion Restrictions, Cites Harassment Providers Face} (L) & Reprod. Right (1, 3), Birth Control (1, 3)\\
\hline
a3-\textit{Warren Is Worth the Headache} (L) & Religious Dom. (2, 5)\\
\hline
a4-\textit{Why Even Pro-Choice Americans Should be Upset with Planned Parenthood} (R) &  Sel. of Fet. Tiss. (6, 7), Sex. Assult Vict. Wom. (-), Wom. Health (-)\\
\hline
a5-\textit{Abusive Abortion Activists Terrorize Children at Pro-Life Rally} (R) & Right of Hum. Life (-)\\
\hline
a6-\textit{A Game Changer for the Abortion Debate} (R) & Right of Hum. Life (-), Sanct. of Life (8, 10), \\
\hline
\end{tabular}}
% \caption{Sample of news articles and associated subframes, each  associated with communities in which they are ranked in top-2 subframes.}
\label{tab:hitmap}
\end{center}
\end{table}
\vspace{-20pt}
\begin{figure}[h]
\centering
\includegraphics[width=0.36\textwidth]{Figures/abortion_article_corr.pdf}
% \caption{Heatmap}
\label{fig:hitmap}
\end{figure}
 

%  For example, community 3, a left leaning community, only has a strong 
 
%  We can analyze the polarity of subframes and politicians observed in the communities and crosscheck the results to validate the community assignment. 

\noindent\textbf{The Political Meaning of Sub-frames} As the analysis above shows, sub-frame code political meaning, as they correspond to talking points typically used by one side to discuss issues. To help analyze this property in a more systematic way, we capture how each sub-frame is used, in either left or right communities. In Figure \ref{fig:subframe-polarity} we plot the average ranking score of each sub-frame in the left biased communities vs. their average ranking score in right biased communities. The analysis demonstrates their political meaning. For example in the context of abortion, the ``sanctity of life'' sub-frame is popular on the right, but barely used on the left, while ``religious domination on women'' has an opposite trend. Note that both have the same parent frame, \texit{morality}, used by both sides.



% The plots are shown in Figure \ref{fig:subframe-polarity}. We can see that in the topic \textit{Abortion}, stance points which are opposing abortion have higher ranking in the right communities, where in the left communities stance points related to women rights and freedom are more highly ranked. The trend is consistent with Republican and Democrat stances in the issue \textit{Abortion}. Note that, "Women health" issue is ranked highest in both type of communities which means it is broader than a polarized stance and discussed in both type of communities. The polarization graph for other two topics are attached in the Appendix section because of space constraint.
  
 
 
% We can see that the articles are closer to the communities according to their bias and the subframe interest of the communities, although they were not included in the communities during embedding learning. This evaluation proves the usefulness of the communities and indicates a way to recommend unshared news articles to the identified communities correctly according to their interest. 




\begin{figure}[ht]
  %\centering
  \begin{subfigure}{\linewidth}
  \centering
  %\includegraphics[width=.48\linewidth]{Figures/abortion_followee_distribution.pdf}
  %\includegraphics[width=.48\linewidth]{Figures/abortion_article_distribution.pdf}\\
  \includegraphics[width=.401\linewidth]{Figures/abortion_followee_rank_corr.pdf}
  \includegraphics[width=.39\linewidth]{Figures/abortion_article_rank_corr.pdf}\\
  \includegraphics[width=.401\linewidth]{Figures/abortion_subframes.pdf}
  \includegraphics[width=.401\linewidth]{Figures/abortion_frames.pdf}\\
  \caption{{\small Abortion}}
   \end{subfigure} %\par\medskip
 \\
   \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.401\linewidth]{Figures/gun_followee_rank_corr.pdf}
  \includegraphics[width=.401\linewidth]{Figures/gun_article_rank_corr.pdf}\\
  \includegraphics[width=.401\linewidth]{Figures/gun_subframes.pdf}
  \includegraphics[width=.401\linewidth]{Figures/gun_frames.pdf}
  \caption{{\small Gun Control}}
   \end{subfigure}%\par\medskip
\\  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=.401\linewidth]{Figures/immigration_followee_rank_corr.pdf}
  \includegraphics[width=.401\linewidth]{Figures/immigration_article_rank_corr.pdf}\\
  \includegraphics[width=.401\linewidth]{Figures/immigration_subframes.pdf}
  \includegraphics[width=.401\linewidth]{Figures/immigration_frames.pdf}
  \caption{{\small Immigration}}
  \end{subfigure}
  \vspace{-10pt}
  \caption{%The top 2 subfigures show the label distribution of followed politicians and shared articles over community ranking.
  Spearman's rank correlation coefficient of communities' ranking of politicians, articles, frames and sub-frames, with the ranking of the leftmost and rightmost community for each topic. }
  
%   Each subfigure shows Spearman's rank correlation coefficient of the ranking of four types of properties inside a community with the rank of the leftmost and rightmost community for each topic. The correlation distribution is shown over community polarity ranking. Upper left graph of each subfigure shows correlation of politicians' ranks, upper right shows correlation of article ranks, lower left shows correlation of subframe ranks and lower right shows correlation of frame ranks. Communities in the blue (left) regions are identified as left communities and in the red (right) regions are identified as right communities.}
  \label{fig:corr}
 \end{figure}


\vspace{-12pt}
% \subsection{Relationship between frames and ideology}
\subsection{Detecting Politically-Segregated Behavior}
The formation of information ``echo-chambers'' is one of the main problems in the way news spreads using social networks. Political segregation inside communities can manifest in multiple ways. The specific articles circulating between members and the identity of political influencers followed by members, are obvious indicators. In addition, we take a deeper look at the content shared, and analyze the frames and sub-frame usage, and their overlap across different communities.   

To capture political segregation in our communities, we take the top left and top right communities, and treat their behavior as the ideal representative of their respective camps, using their ranking for each one of the four indicators. We compare these rankings with those of each one of the communities using Spearman's rank correlation coefficient. The change in correlation of ranking by community ranking are shown in Figure \ref{fig:corr} for the three topics\footnote{We exclude two ``Gun Control'' communities , which had extremely low sharing and following behaviour compared to the others (e.g., $14$ articles compared to the average of $470$)}. Using this analysis, the ``perfect'' echo-chamber behavior would correspond to a correlation of 1, between the ranking of communities with the same political label as the ideal ranking, and -1 when the labels do not match.  Looking at the results, communities with a strong political bias indeed demonstrate this trend, in all four indicators, across all three topics. However, as the communities get closer to the center, the trend is different. The difference in correlation between these communities' ranking and top-left and right ranking decreases, indicating that in these communities both perspectives are represented, and their members are influenced by politicians from both sides. Finally, comparing the correlations for frames vs. sub-frames demonstrates the importance of the latter. When comparing the top-left and right communities, the inverse correlation between their sub-frames ranking is higher compared to the frames.

% Now, to observe the homophily in share, follow behaviour and subframe, frame usage we compare the ranking of politicians, news articles, subframes, frames inside each community with the leftmost and rightmost communities (according to the community rank we defined). The change in correlation of ranking by community ranking are shown in Figure \ref{fig:corr} for the three topics\footnote{We exclude two ``Gun Control'' communities , which had extremely low sharing and following behaviour compared to the others (e.g., $14$ articles compared to the average of $470$)}.


% We can see from the graphs that, the correlation of ranking of politicians, news articles, subframes and frames decrease as we go from leftmost community to righmost community. That means communities are polarized in their follow, share behaviours and in the way they frame a topic. We can see from the figures that, the decrease of correlation in subframe rank is higher than the decrease of correlation in frame ranking which supports our claim that frame usage cannot strongly represent political polarization.     


% (e.g., $14$ articles shared , follow $51.5$ politicians on average while the other communities share $470.18$ news articles and follow $342.27$ politicians on average. So, we exclude them from the correlation graphs as outliers.


 

==> 5Experiments_new.tex <==
\section{Experiments}
{\color{red}{Are there results from the previous paper that should move here? Some of the qualitative analysis at the document level seems relevant}}

